On Train-Test Class Overlap and Detection for Image Retrieval

How important is it for training and evaluation sets to not have class overlap in image retrieval? We revisit Google Landmarks v2 clean, the most popular training set, by identifying and removing class overlap with Revisited Oxford and Paris [34], the most popular evaluation set. By comparing the original and the new RGLDv2-clean on a benchmark of reproduced state-of-the-art methods, our findings are striking. Not only is there a dramatic drop in performance, but it is inconsistent across methods, changing the ranking.What does it take to focus on objects or interest and ignore background clutter when indexing? Do we need to train an object detector and the representation separately? Do we need location supervision? We introduce Single-stage Detect-to-Retrieve (CiDeR), an end-to-end, single-stage pipeline to detect objects of interest and extract a global image representation. We outperform previous state-of-the-art on both existing training sets and the new RGLDv2-clean. Our dataset is available at https://github.com/dealicious-inc/RGLDv2-clean.

==> exp/datasets.tex <==







==> exp/exp_abl.tex <==

SfM-120k



SfM-120k



SfM-120k








SfM-120k

\begin{table}[t]
%\vspace{-5pt}
%\vspace{5pt}
\centering
\scriptsize
%\tiny
%\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{l*{7}{c}} \toprule
\mr{2}{\Th{Dim}} & \mr{2}{\Th{Oxf5k}} & \mr{2}{\Th{Par6k}} & \mc{2}{\Th{Medium}} & \mc{2}{\Th{Hard}} \\ \cmidrule(l){4-7}
 & & &  \rox & \rpa & \rox & \rpa \\ \midrule
4096 & 87.8 & 90.2 & 64.8 &  76.8 & 38.1 & 52.8 \\
3097 & 89.8 & 90.5 & \tb{67.4} &  76.9 & \tb{42.5} & 53.0 \\
2048 & \tb{89.9} & \tb{92.0} & {67.3} &  {\tb{79.4}}& {{42.4}} & {\tb{57.5}}\\ 
1024 & 88.9  & 91.2  & 65.7 &  76.7 & 40.1 & 52.0 \\
512  & 85.3  & 89.2  & 61.9 &  74.4 & 36.5 & 48.9 \\
\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{mAP comparison of different N features dimension in our model.}
\label{tab:scm}
\end{table}







==> exp/exp_gldv2_clean3.tex <==
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
%\def\arraystretch{1.13}%  1 is the default, row height
{
\centering
%\footnotesize
\scriptsize
%\setlength\extrarowheight{-1pt}
%\setlength{\tabcolsep}{0pt}
\setlength{\tabcolsep}{0.8pt}
%\resizebox{\textwidth}{!}
{
\begin{tabular}
{@{~}L{4.1cm}C{0.03cm}C{0.03cm}C{0.03cm}L{0.03cm}|C{\cw}C{\cw}|C{\cw}C{\cw}C{\cw}C{\cw}|C{\cw}C{\cw}C{\cw}C{\cw}|C{\cw}C{\cw}}
	\toprule
	\multicolumn{5}{@{~}c|}{\multirow{3}{*}{\Th{Method}}} &	
        \multicolumn{2}{c|}{\Th{Base}}   & 
        \multicolumn{4}{c|}{\Th{Medium}} & 
        \multicolumn{4}{c|}{\Th{Hard}}    &
        \multicolumn{2}{@{~}c}{\multirow{3}{*}{\Th{Mean}}}   \\
	\cmidrule{6-15}
	& & & & & {\fontsize{7}{6}\selectfont \oxf5k}  & {\fontsize{7}{6}\selectfont \paris6k} &
 \multicolumn{2}{c}{{\fontsize{7}{6}\selectfont \rox}} &
 \multicolumn{2}{c}{{\fontsize{7}{6}\selectfont \rpa}} & 
 \multicolumn{2}{c}{{\fontsize{7}{6}\selectfont \rox}} & 
 \multicolumn{2}{c|}{{\fontsize{7}{6}\selectfont \rpa}} \\
        & & & & & \tiny mAP &  \tiny mAP &  \tiny mAP & \tiny mP@10 &  \tiny mAP & \tiny mP@10 &  \tiny mAP & \tiny mP@10 &  \tiny mAP & \tiny mP@10 \\
\midrule
    %\rowcolor{lightgray}
    %\midrule
    %\rowcolor{lightgray2}
    %\multicolumn{23}{c}{\Th{GLDV3-Clean}} \\ \midrule
    %ep20
    %\rowcolor{lightgray2}
    %ep1
    Yokoo~\etal~\cite{Yokoo01}$^\dagger$ (Base)             & & & & & 86.1   & 93.9     & 64.5 & 81.0 & 84.1 & \tb{95.4} & 35.6 & 51.5 & \tb{68.7} & 86.4 & 74.1    \\ 
    SOLAR~\cite{Ng01}$^\dagger$               & & & & & 90.6     & \tb{94.4} & 70.8     & 84.6 & 80.3 & 94.6 & 48.0 & \tb{62.3} & 61.8 & 83.9 & \tb{79.3}    \\  
    %ep11 
    GLAM~\cite{SCH01}$^\ddagger$              & & & & & \tb{90.9} & 94.1     & \tb{72.2} & 84.7 & 83.0 & 95.0 & \tb{49.6} & 61.6 & 65.6 & \tb{87.6} & 78.3 \\    
    DOLG~\cite{yang2021dolg}$^\dagger$        & & & & & 88.3      & 93.9     & 70.8 & \tb{85.3} & \tb{83.2} & \tb{95.4} & 47.4 & 60.0 & 67.9 & 87.4 & 78.6  \\ 
    % ep17? 모델이 없다.ㅠㅠ
    %Token~\cite{tokens}$^\dagger$             & & & & & 84.3      & 90.0     & 61.4 & 76.4 & 75.8 & 94.0 & 36.9 & 55.2 & 54.4 & 81.0 & 70.8  \\
    % ep19
    Token~\cite{tokens}$^\dagger$             & & & & & 81.2      & 89.6     & 60.8 & 77.7 & 75.8 & 94.3 & 37.3 & 54.1 & 54.8 & 81.3 & 70.8  \\ 
    %\rowcolor{lightgray}
    \midrule
    %\rowcolor{lightgray2}
    %\multicolumn{17}{c}{\Th{Ours}} \\ \midrule
    % ep8
    %SCH-R101-V12-4-28   & & & & & 93.0  & 93.1 & 74.7 &  87.7 & -- & -- & 82.9 & 96.3  & -- & -- & 54.2  & 66.6 & -- & -- & 65.2 & 86.9 & -- & -- \\
    % ep15
    %SCH-R101-V12-4-28   & & & & & 90.0 & 94.0 & 71.3 & 85.7 & -- & -- & 82.2 & 96.4 & -- & -- & 52.6 & 65.4 & -- & -- & 65.6 & 87.0 & -- & -- \\
    %SCH-R101-V12-4-28   & & & & & 91.1 & 93.8 & 72.4 & 84.9 & 83.7 & 96.1 & 52.9 & 65.6 & 66.0 & 87.6  \\
    %SCH-R101-V12-4-28-NW   & & & & & 89.8 & \tb{94.6} & \tb{73.7} & \tb{85.5} & \tb{84.6} & \tb{96.7} & \tb{54.9} & \tb{66.6} & \tb{68.5} & \tb{89.1} & \tb{80.0} \\
    % eval_train_v12_4_28_gdv2_filtered_nowarmup_ep8.log
    $\mathbf{S_{2}D2R}$ (Ours)   & & & & & 89.8 & \ok{\tb{94.6}} & \ok{\tb{73.7}} & \ok{\tb{85.5}} & \ok{\tb{84.6}} & \ok{\tb{96.7}} & \ok{\tb{54.9}} & \ok{\tb{66.6}} & \ok{\tb{68.5}} & \ok{\tb{89.1}} & \ok{\tb{80.0}} \\ 
    %ep15
    %$\mathbf{S_{2}D2R}+FT$ (Ours)   & & & & & 90.3 & \tb{95.6} & \tb{76.7} & \tb{87.1} & \tb{87.4} & \tb{96.3} & \tb{60.8} & \tb{71.1} & \tb{74.7} & \tb{90.9} & -- \\ 
     %ep7
    $\mathbf{S_{2}D2R}$+FT (Ours)   & & & & & \red{\tb{90.9}} & \red{\tb{96.1}} & \red{\tb{77.8}} & \red{\tb{88.0}} & \red{\tb{87.4}} & \red{\tb{97.0}} & \red{\tb{61.9}} & \red{\tb{70.4}} & \red{\tb{75.3}} & \red{\tb{90.0}} & \red{\tb{83.6}} \\ 
    %SCH-R101-V12-4-28-NW   & & & & & 91.1 & 94.6 & 73.7 & 85.5 & 84.6 & 96.7 & 54.9 & 66.6 & 68.5 & 89.1  \\
 \bottomrule
 \end{tabular}
}
}


==> exp/sup_exp.tex <==
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\def\arraystretch{1.13}%  1 is the default, row height


{
\centering
\footnotesize
\setlength\extrarowheight{-1pt}
\setlength{\tabcolsep}{0pt}
\resizebox{\textwidth}{!}
{
\begin{tabular}
{@{~}L{4.1cm}C{0.03cm}C{0.03cm}C{0.03cm}L{0.03cm}|C{\cw}C{\cw}C{\cw}C{\cw}C{\cw}C{\cw}C{\cw}C{\cw}|C{\cw}C{\cw}C{\cw}C{\cw}C{\cw}C{\cw}C{\cw}C{\cw}}
	\toprule
	\multicolumn{5}{@{~}c|}{\multirow{3}{*}{\Th{Method}}} & \multicolumn{4}{c|}{\Th{Medium}} & \multicolumn{4}{c}{\Th{Hard}} \\
	\cmidrule{4-13}
	& & & & &  
 \multicolumn{1}{c}{{\fontsize{7}{6}\selectfont \rox}} &
 \multicolumn{1}{c}{{\fontsize{7}{6}\selectfont \rox+\r1m}} & 
 \multicolumn{1}{c}{{\fontsize{7}{6}\selectfont \rpa}} &
 \multicolumn{1}{c}{{\fontsize{7}{6}\selectfont \rpa+\r1m}} &
 \multicolumn{1}{c}{{\fontsize{7}{6}\selectfont \rox}} &
 \multicolumn{1}{c}{{\fontsize{7}{6}\selectfont \rox+\r1m}} & 
 \multicolumn{1}{c}{{\fontsize{7}{6}\selectfont \rpa}} &
 \multicolumn{1}{c}{{\fontsize{7}{6}\selectfont \rpa+\r1m}} \\
	& & & & & \tiny mAP & \tiny mAP & \tiny mAP & \tiny mAP & \tiny mAP & \tiny mAP & \tiny mAP & \tiny mAP \\
	\midrule
	\rowcolor{lightgray2}
	\multicolumn{13}{c}{\Th{Global Descriptors (SfM-120k)}} \\ \midrule
 % RITAC18
GeM-R101~\cite{Radenovic01}       & & & & & 64.7 & 45.2 & 77.2 & 52.3 & 38.5 & 19.9 & 56.3 & 24.7 \\
%
AGeM-R101~\cite{gu2018attention} & & & & & \tb{67.0} & -- & \tb{78.1} & --  &\tb{40.7} & -- & \tb{57.3} & --    \\
%
GLAM-R101~\cite{SCH01}          & & & & &  66.2 & -- & 77.5 & -- &39.5 & -- & 54.3 & -- \\
 
%\midrule
%\rowcolor{lightgray2}
%\multicolumn{23}{c}{\Th{SCH Exp  (SfM-120k)}} \\ \midrule
%R101-V12-4-22 : add fc-ep29 & & & & & \red{\tb{89.8}} & {92.0} & \red{\tb{67.1}} & \red{\tb{84.7}} & \red{\tb{50.2}} & \red{\tb{76.1}} & \red{\tb{79.3}} & 98.0  & 51.3 & 95.3 & \red{\tb{42.0}} & \red{\tb{55.6}} & \red{\tb{22.5}} & \red{\tb{35.9}} & \red{\tb{57.3}} & 86.4  & 22.2 & 69.0  \\
%
% R101-V12-4-22 : add fc-ep33 & & & & & \red{\tb{89.7}} & {92.0} & \red{\tb{67.0}} & 84.2 & \red{\tb{49.9}} & \red{\tb{75.7}} & \red{\tb{79.4}} & \red{\tb{98.3}}  & 51.5 & \red{\tb{95.6}} & \red{\tb{41.0}} & \red{\tb{54.4}} & \red{\tb{22.0}} & 34.7 & \red{\tb{57.4}} & 86.7  & 22.4 & 69.3  \\
R101-V12-4-28 : ep30  & & & & & \red{\tb{67.3}}& \red{\tb{50.3}} & \red{\tb{79.4}} & 51.4 &  \red{\tb{42.4}} & \red{\tb{22.4}} & \red{\tb{57.5}}& 22.4  \\
%R101-V12-4-28 : ep30  & & & & & \red{\tb{89.9}} & {92.0} & \red{\tb{67.3}}& \red{\tb{85.1}} & \red{\tb{50.3}} & \red{\tb{75.5}} & \red{\tb{79.4}} & 97.9  & 51.4 & \red{\tb{95.7}} & \red{\tb{42.4}} & \red{\tb{56.4}} & \red{\tb{22.4}} & \red{\tb{35.9}} & \red{\tb{57.5}} & 87.1  & 22.4 & 69.4 \\
%R101-V12-4-28 : ep54  & & & & & {89.6} & {91.9} & \red{\tb{67.1}}& \red{\tb{84.7}} & \red{\tb{50.2}} & \red{\tb{75.8}} & \red{\tb{79.4}} & \red{\tb{98.1}}  & 51.3 & \red{\tb{95.6}} & \red{\tb{42.1}} & \red{\tb{56.0}} & \red{\tb{22.4}} & \red{\tb{35.4}} & \red{\tb{57.3}} & 86.9  &22.2 & 69.9 \\
\midrule

%GLAM-R101~\cite{SCH01} - GLDV3 ep15   & & & & & 86.8 & 91.8 & 64.2 & 77.7 & -- & -- & 77.4 & 92.3 & -- & -- & 40.7 & 54.6 & -- & -- & 58.9 & 82.7 & -- & --   \\
%\midrule
%\rowcolor{lightgray}
%	\multicolumn{23}{c}{\Th{GLDV1 } } \\ \midrule
%SOLAR~\cite{Ng01}       & & & & & -- & -- & 69.9 & 86.7 & 53.5 & 76.7  & 81.6 & 97.1 & 59.2 & 94.9 & 47.9 & 63.0 & 29.9 & 48.9 & 64.5 & 93.0 &  33.4 & 81.6 \\

 \bottomrule
 \end{tabular}
}
}

==> tex/sec_conclusion-1.tex <==
\section{Conclusion}
\label{sec:conclusion}

This study was initiated with dual motivations and consequently identified a particular problem, for which it outlined a series of solutions. The study encountered two primary challenges corresponding to these motivations. First, within the range of training datasets in the ILIR field—including NC-clean, SfM-120k, and GLDv2-clean—the GLDv2 presented an issue of overlapping landmarks with the evaluation set. Second, on the algorithmic front, D2R methods have generally been based on two-stage pipeline methods. These are inherently inefficient, as they lack an end-to-end learning framework and include an additional object detection phase. To tackle these issues, we introduced a revamped dataset, $\cR$GLDv2-clean, as an improvement over GLDv2-clean. We also proposed a single-stage pipeline learning method, dubbed \ours, designed for efficient and effective end-to-end learning. Notably, \ours achieves SOTA performance, not only on established training sets such as NC-clean and SfM-120k but also on the newly released \emph{$\cR$GLDv2-clean} dataset.

% 우리 연구는 두개의 Motivation에서 시작되었고, 이 과정에서 문제점을 정의하고 이를 해결하기 위한 방법들에 대해 기술하였다. 
% 두개의 Motivation에는 두가지 문제가 있었다. 첫번째, ILIR 분야에서 학습셋으로 사용하고 있는 NC-clean, SfM-120k, GLDV2-clean 데이터셋중에서, GLDV2-clean은 evaluation set과 오버래핑된 랜드마크가 존재하는 문제점이 있었다. 
% 두번째, 알고리즘 측면에서 일반적으로 $\mathbf{D2R}$ 방법은 2-Stage Pipeline 방법이었는데, 이는 Object Detection 파트가 추가되는 End-to-End 방법이 아니어서 비효율적인 문제가 있었다. 
% % 두개의 Motivation에 대해서, 첫번째, ILIR분야에서 학습셋으로 사용하고 있는 NC-clean, SfM-120k, GLDV2-clean 데이터셋중에서, NC-clean와 SfM-120k와는 달리 GLDV2-clean은 evaluation set과 오버래핑된 랜드마크가 존재하는 문제점이 있었고, 
% % 두번째, 알고리즘 측면에서 일반적으로 $\mathbf{D2R}$ 방법은 2-Stage Pipeline 방법이었는데, 이는 Object Detection 파트가 추가되는 End-to-End 방법이 아니어서 비효율적인 문제가 있었다. 
% 최종적으로, 이를 해결하기 위해 우리는 GLDV2-clean를 수정한 새로운 데이터셋 (\emph{$\cR$GLDV2-clean})을 공개하였다. 
% 그리고 end-to-end 학습이 가능한 single-stage Pipeline 학습 방법 (\ours)을 제안하여 이 효능적이고 효과적인 방법에 대해 기술하였다. 
% % 그리고, 1-Stage Pipeline 방법인 End-to-End 학습 방법 (\ours)을 제안하여 이 효능적이고 효과적인 방법에 대해 기술하였다.
% 또한, 우리가 제안한 \ours은 기존 학습셋인 NC-clean, SfM-120k 뿐만아니라, 새롭게 공개한 \emph{$\cR$GLDV2-clean}에서도 SOTA 성능을 보였음을 입증하였다. 
 


==> tex/sec_dataset-1.tex <==
%\subsection{Two-Stage vs. Single-Stage pipeline for Detected to Retrieval}
\vspace{-5pt}
\section{Revisiting Goolge landmark Dataset V2}
\label{sec:RevisitingGLDV2}

\vspace{-3pt}
\paragraph{Unfaired Landmark Clean Trainset}
A key feature of current landmark datasets in the field of ILIR is their fragmented origins: training and evaluation sets are often independently collected and released by different studies. Initial datasets contained tens of thousands of images, a number that has now swelled into the millions. Evaluation sets such as Oxford5k (\oxf5k)~\cite{Philbin01} and Paris6k (\paris6k)~\cite{Philbin02}, and their more recent versions, Revisited Oxford (\roxf~or \rox) and Paris (\rpar~or \rpa)~\cite{RITAC18}, are commonly used. Concurrently, training sets such as  \emph{Neural Code} (NC)~\cite{Babenko01}, \emph{Neural Code clean} (NC-clean)~\cite{Gordo01}, SfM-120k~\cite{Radenovic01}, Google Landmarks V1 (GLDv1)~\cite{delf}, and Google Landmarks V2 (GLDv2 and GLDv2-clean)~\cite{Weyand01} have been sequentially introduced and are widely applied in related studies.
The \emph{Clean} versions of these datasets are curated based on two main criteria. First, they are collected through text-based keyword searches on platforms such as Google. Second, they are filtered to remove any landmarks that overlap with those in evaluation sets like \oxf5k and \paris6k. The first criterion often results in a mix of \emph{Noisy} images in addition to images containing specific landmarks, called the noisy dataset. Typical \emph{Noisy} datasets are NC, GLDv1, and GLDv2. To solve this problem, the classes are filtered in various ways~\cite{Gordo01, Radenovi01} to ensure that they contain only the same landmark (instance), which is called the clean dataset. Representative clean datasets include NC-clean, SfM-120k, and GLD-v2-Clean. They are widely used as regular training sets. Interestingly, while NC-clean and SfM-120k adhere to both criteria, Google Landmarks V2 Clean falls short of the second criterion. This discrepancy has been acknowledged not only in this study but also in various other previous studies~\cite{superfeatures} and broader community\footnote{\url{https://github.com/MCC-WH/Token/issues/1}} discussions. This means that it is not fair to compare studies using Google Landmarks V2 Clean with those that utilize NC-clean or SfM-120k for training. Studies using the GLDv2-clean training set may show artificially \emph{inflated accuracy} levels during testing. 
Our study aims to address this problem and describes the remedial methodology, where we also introduce a newly modified dataset.

\vspace{-5pt}
\paragraph{Confirming Overlapping Landmarks}
First, it is necessary to verify whether common landmark categories exist between the training and evaluation sets. In this study, we employ the GLAM~\cite{SCH01} algorithm to extract image features from the training sets GLDv2-clean, NC-clean, and SfM-120k, as well as the evaluation sets \oxf5k and \paris6k. These extracted features from GLDv2-clean are then indexed using the Approximate Nearest Neighbor (ANN)\footnote{\url{https://github.com/kakao/n2}} search method. Subsequently, the evaluation sets \oxf5k and \paris6k are used as query sets to perform ANN indexing on each of the aforementioned training sets. \autoref{fig:fig2} displays the results. The green box (on the left) represents the outcome when using \oxf5k as a query, while the blue box (on the right) indicates the result with \paris6k. The red box in both sets highlights the query used for input. Each row represents the result of applying ANN indexing to the query using data from GLDv2-clean, NC-clean, and SfM-120k. The columns display the top-5 ranking results. The pink box identifies images with landmarks that match those in the query. Interestingly, none of the results from NC-clean and SfM-120k feature landmarks that resemble the query. In contrast, the results from GLDv2-clean include images with landmarks identical to those in the query. This suggests that using the GLDv2-clean dataset could lead to artificially \emph{inflated accuracy} scores in testing when compared to NC-clean and SfM-120k. Given the unfairness of this comparison, the validity of previous studies that employed the GLDv2-clean dataset should be reconsidered.

\vspace{-10pt}
\paragraph{Verification} These GLDv2-clean ranking results are filtered through two verification steps. First, for an automatic verification process, SIFT is used~\cite{Lowe01}. LDs are extracted for results up to top-k and matched using kd-tree. For the matching results, RANSAC is used to eliminate outliers (false matching) to determine the final match. Class information global identifiers (GIDs) from the GLDv2-clean dataset is used to exclude only the most matched GIDs from the final matching results. Second, since the above process can sometimes include false matching, three reviewers manually check the first results above for final verification. \autoref{fig:figa1} illustrates this process. Moreover, text queries from GLDv2-clean, Oxford5k, and Paris6k were scrutinized. Where, for one and the same matched query (\emph{Hotel des Invalides Paris}), all images contained in the GID were removed, with or without the above validation steps.

\begin{figure}[t]
\centering\includegraphics[width=0.95\columnwidth]{fig/A1.png}
%\end{center}
\vspace{-12pt}
   \caption{ Filtering pipelines for Clean Dataset 
   }
\label{fig:figa1}
\end{figure}
%
%
\vspace{-10pt}
\paragraph{Revisiting GLDV2-clean ($\cR$GLDV2-clean)} Through the above two steps, a revised GLDv2-clean dataset, \emph{$\cR$GLDV2-clean}, was generated. \autoref{tab:table1} presents the statistical values of the filtered data. In this table, \roxf and \rpar have 36 and 38 overlapping landmarks out of 70, respectively, which equates to a duplication rate of approximately 51\% and 54\%, respectively. This is a very large percentage, as the duplication rate is over half for both evaluation sets. In other words, this reaffirms the inherent issue with GLDv2-clean once more. The new dataset eliminates 1,565 images contained within 17 GIDs from GLDv2-clean. \autoref{tab:table2} compares the statistical numbers for the existing clean datasets and the \emph{$\cR$GLDV2-clean} of this study.
\emph{Based on this, previous studies that applied GLDv2-clean were excluded. For a fairer study, only those previous studies that used clean training sets (NC-clean, SfM-120k, {$\cR$GLDV2-clean}).}% rather than the existing noisy sets were compared.}

\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{3.2pt}
\begin{tabular}{lcccc} \toprule
\Th{Eval} & \Th{\#Eval Img} & \Th{\#dupl Eval} & \Th{\#dupl gldv2 GID} & \Th{\#dupl gldv2 Img} \\\midrule
\rox & 70 & 36 (51\%) &  10 & 1227 \\
\rpa & 70 & 38 (54\%)  &  7 & 315 \\
\Th{text} &  &  &  1  & 23 \\
\midrule
\Th{total} & 140 & 74  & 17 & 1565 \\
\bottomrule
\end{tabular}
\vspace{-8pt}
\caption{Statistical information about duplicate images/categories with (\roxf, \rpar) and GLDV2. \Th{Eval}:Evaluation Sets. \Th{dupl}:duplicated. \Th{img}:Image. \Th{GID}:GLDV2 category. }
\label{tab:table1}
\end{table}
%
%
\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{15.5pt}
\begin{tabular}{lcc} \toprule
\Th{Train Set} & \Th{\#Images} & \Th{\#Classes} \\ \midrule
%NC-noisy & 213,678 & 672 \\
NC-clean & 27,965 & 581 \\
SfM-120k & 117,369 & 713 \\
%GLDv1-noisy & 1,225,029  &  14, 951 \\
%GLDv2-noisy & 4,132,914  &  203,094 \\
GLDv2-clean & 1,580,470 & 81,313 \\
\midrule
\tb{\emph{$\cR$GLDV2-clean} (ours)} &  1,578,905 & 81,296 \\
%ours-clean & 513,768 & 156,331 \\
%ours-clean$\ge15$ & 101,285 & 2,430 \\
\bottomrule
\end{tabular}
\vspace{-8pt}
\caption{Statistics of Clean-DataSests}
\label{tab:table2}
\end{table}

==> tex/sec_dataset-2.tex <==
\section{Revisiting Google Landmarks v2}
\label{sec:dataset}

%------------------------------------------------------------------------------
\begin{figure*}[t]
\centering
\fig[0.95]{2}
\vspace{-6pt}
\caption{Confirming overlapping landmark categories between training sets (GLDv2-Clean, NC-Clean, SfM-120k) and evaluation sets (Oxford5k, Paris6k). Green box (left): \roxf; blue box (right): \rpar. Top row: GLDv2-clean; middle row: NC-clean; bottom row: SfM-120k. Red box: query image. The query image from the evaluation set in each box/row is followed by top-5 most similar images from the training set. Pink box: training image landmark identical with query (evaluation) image landmark.
More examples can be found in the Appendix.
%(\autoref{fig:fig2_sup}).
\CH{I can't do this for each image. Top5 was generated by a randomized code as a result. Therefore, I generated 6 pdfs with one result each. (2\_*\_*.pdf)}
\iavr{Thanks, 6 pdf is still ok, but there are no pink boxes in the 6 pdf. I could add them myself in Latex if each image was separate, but I cannot do anything now. Can you create again with pink boxes? Can you also add a bit of space between images and a little more space between query and retrieved? As I said, PDFs are not needed here. They can be png/jpg.}
}
\label{fig:fig2}
\end{figure*}
%------------------------------------------------------------------------------

\paragraph{Motivation}

A key weakness of current landmark retrieval datasets is their fragmented origins: training and evaluation sets are often independently collected and released by different studies. Initial datasets contained tens of thousands of images, a number that has now grown into the millions.

\emph{Evaluation sets} such as Oxford5k (\oxf5k)~\cite{Philbin01} and Paris6k (\paris6k)~\cite{Philbin02}, as well as their more recent versions, Revisited Oxford (\roxf~or \rox) and Paris (\rpar~or \rpa)~\cite{RITAC18}, are commonly used for benchmarking. Concurrently, \emph{training sets} such as \emph{Neural Codes} (NC)~\cite{Babenko01}, \emph{Neural Codes clean} (NC-clean)~\cite{Gordo01}, SfM-120k~\cite{Radenovic01}, Google Landmarks v1 (GLDv1)~\cite{delf}, and Google Landmarks v2 (GLDv2 and GLDv2-clean)~\cite{Weyand01} have been sequentially introduced and are widely used for representation learning.

These training sets are typically curated according to two criteria: first, to depict particular landmarks, and second, to not contain landmarks that overlap with those in the evaluation sets. They are originally collected by text-based web search using particular landmark names as queries. This often results in \emph{noisy} images in addition to images depicting the landmarks. Thus, NC, GLDv1 and GLDv2 are \emph{noisy} datasets. To solve this problem, images are filtered in different ways~\cite{Gordo01, Radenovi01} to ensure that they contain only the same landmark (instance). Accordingly, NC-clean, SfM-120k, and GLDv2-clean are \emph{clean} datasets.

The \emph{clean} datasets are also typically filtered to remove overlap with the evaluation sets. However, while NC-clean and SfM-120k adhere to both criteria, GLDv2-clean falls short of the second criterion. This discrepancy is not a limitation of GLDv2-clean per se, because the dataset comes with its own split of training, index and query images. However, the community is still using the \roxf and \rpar evaluation sets, whose landmarks have not been removed from GLDv2-clean. Besides, landmarks are still overlapping between the GLDv2-clean training and index sets.

This discrepancy is particularly concerning because GLDv2-clean is the most common training set in state-of-the-art studies. It has been acknowledged in previous work~\cite{superfeatures} and in broader community discussions\footnote{\url{https://github.com/MCC-WH/Token/issues/1}}. The effect is that results of training on GLDv2-clean are not directly comparable with those of training on NC-clean or SfM-120k. Results on GLDv2-clean may show artificially \emph{inflated performance}. This is often attributed to its larger scale but may in fact be due to overlap. Our study aims to address this problem by introducing a new version of GLDv2-clean.

%------------------------------------------------------------------------------

\paragraph{Identifying overlapping landmarks}

First, it is necessary to confirm whether common landmark categories exist between the training and evaluation sets. We extract image features from the training sets GLDv2-clean, NC-clean, and SfM-120k, as well as the evaluation sets \rox and \rpa. The features of the training sets are then indexed and the features of the evaluation sets \rox and \rpa are used as queries to search into the training sets.

\autoref{fig:fig2} displays the results. Interestingly, none of the retrieved images from NC-clean and SfM-120k training sets depict the same landmark as the query image from the evaluation set. By contrast, the top-5 most similar images from GLDv2-clean all depict the same landmark as the query. This suggests that using GLDv2-clean for training could lead to artificially \emph{inflated performance} during evaluation, when compared to NC-clean and SfM-120k. Since such comparison is unfair, the validity of previous studies that use GLDv2-clean for training should be reconsidered.

%------------------------------------------------------------------------------
\begin{figure}[t]
\centering
\fig[.95]{f3.pdf}
\vspace{-6pt}
\caption{Ranking and verification pipeline to remove landmark categories from GLDv2-clean that overlap with those of the \rox and \rpa evaluation sets and obtain the revisited version, $\cR$GLDv2-clean. \iavr{Please, NC-Clean $\to$ NC-clean and GLDV2-Clean $\to$ GLDv2-clean, everywhere. I am doing this in the text but I cannot do figures.} 
\CH{I fixed it to your request. 
And similarly, I've written how to create the figure in SLACK. 
Is this the resolution you want?}}
\label{fig:figa1}
\end{figure}
%------------------------------------------------------------------------------

\paragraph{Verification}

Now, focusing on GLDv2-clean training set, we retrieve images for each query image from the evaluation set as above and we filter the top-$k$ ranked images by two verification steps. First, we automatically verify that the same landmark is depicted by using robust spatial matching on correspondences obtained by local features and descriptors. \alert{We only keep those visual matches for which the landmark category as specified by a global identifier (GID) also matches the landmark name in the evaluation set.} \iavr{Is this correct?} \CH{I proceeded regardless of the \emph{name} of the landmark.: GIDs can be thought of as the names of landmarks. However, I didn't take landmark names into account.} \iavr{Then, what does ``text'' mean in \autoref{tab:table1}? Isn't it the landmark name? Also, what do we do if not what I say here? The original says ``Class information global identifiers (GIDs) from the GLDv2-clean dataset is used to exclude only the most matched GIDs from the final matching results.'' I cannot follow this at all. Does it mean the same as my sentence below ``For every match between a query from the evaluation set and an image from GLDv2-clean, the entire landmark category from the corresponding GID is removed?''}
\CH{I answered the question below, and wrote about it in Slack. We were stumped. "Hotel des Invalides Paris" and the same landmark title in the training and evaluation sets, but the visual matching was failing.
We thought this could be a possible problem (false positive verification), and since there were only a few images, we decided it would be fine to remove this GID. Were we wrong?}

Second, since automatic verification may fail, three human evaluators manually check all matches obtained in the first step. We only keep matches that are confirmed by at least one human evaluator. \iavr{I didn't ask before, but is this correct? At least one human?} \CH{SIFT matching has many "false matchings".
So, we double-checked the actual top-k results (global descriptors) and the verficiation results with three different people.}For every match between a query from the evaluation set and an image from GLDv2-clean, the entire landmark category from the corresponding GID is removed. \autoref{fig:figa1} illustrates the complete ranking and verification process.

\alert{Moreover, text queries from GLDv2-clean, Oxford5k, and Paris6k were scrutinized. Where, for one and the same matched query (\emph{Hotel des Invalides Paris}), all images contained in the GID were removed, with or without the above validation steps.} \iavr{This is unclear. Are GIDs used to filter visual matches as specified above? If so, why are GID are used alone, without visual matching? Does ``Invalides'' not yield any visual matches and needs to be handled by text alone?}
\CH{We considered visually matching in time first.
But we decided to remove all images within the matching GID. 
We didn't want to introduce any unnecessary problems (e.g., if by mistake, something should have been removed but wasn't). 
We checked to see if there were any cases where the landmark names were exactly the same, and there was one, and again, to avoid causing unnecessary problems, we decided to remove them all, regardless of temporal matching.We also realized that the number of images in all the GIDs we wanted to remove was very small, so we thought it was okay.}
\iavr{``Temporal matching'' is unclear to me, but let me see if I get this right. There is a landmark name for each GID but you didn't use them, unless there was an exact match with the test set. The only case was ``Hotel des Invalides Paris'' and this is the ``Text'' row in \autoref{tab:table1}. Everything else is based on visual matching and human verification only. Correct? But then again, see my question above: Does ``Invalides'' not yield any visual matches? Because if it does, then we do not need to complicate things by talking about ``Text''. We can say that everything is based on visual matching. This is also consistent with \autoref{fig:figa1}, which does not say anything about ``Text''.}
\CH{right!! I added it to fig.3.  
I think this is getting too complicated!
Just for simplicity, besides the visual matching, I only added the GLDV2-Clean landmark titles and the one matching the title "paris and oxford" as targets for removal. (added to the figure).
"temporal matching" is my mistake. I'm sorry, my mistake, and my understanding of your comments on this part was not good enough.}
%------------------------------------------------------------------------------
\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{3.2pt}
\begin{tabular}{lcccc} \toprule
\Th{Eval} & \Th{\#Eval Img} & \Th{\#Dupl Eval} & \Th{\#Dupl GLDv2 GID} & \Th{\#Dupl GLDv2 Img} \\\midrule
\rox & 70 & 36 (51\%) &  10 & 1227 \\
\rpa & 70 & 38 (54\%) &   7 & 315 \\
Text &  &  &  1  & 23 \\ \midrule
Total & 140 & 74  & 18 & 1565 \\
\bottomrule
\end{tabular}
\vspace{-6pt}
\caption{Statistics of GLDv2-clean training images / landmark categories that overlap (are duplicate) with \rox and \rpa evaluation sets and are removed in our $\cR$GLDv2-clean. \Th{Eval}: evaluation sets; \Th{Dupl}: duplicated; \Th{GID}: GLDv2 category; \Th{Img}: image. \iavr{We need to provide the names of GIDs in the Appendix.} \CH{GIDs: 6190, 19172, 28949, 37135, 42489, 44923, 47378, 69195, 138332, 144472, 145268, 146388, 147275, 152496, 167104, 167275, 181291, 192090 - I will double-check before submission.} \iavr{But, each GID also has a landmark name, right? Then, for each one of the 18 removed classes, report GID (number), landmark name from GLDv2-clean, landmark name from Oxford/Paris and which test set it overlaps (Oxford or Paris). That's a table with 4 columns, to be added in the Appendix. Can you do that?} \CH{I'll let you know when I finalize this.}}
\label{tab:table1}
\end{table}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}
\centering
\scriptsize
% \setlength{\tabcolsep}{15.5pt}
\begin{tabular}{lcc} \toprule
\Th{Training Set} & \Th{\#Images} & \Th{\#Categories} \\ \midrule
%NC-noisy & 213,678 & 672 \\
NC-clean & 27,965 & 581 \\
SfM-120k & 117,369 & 713 \\
%GLDv1-noisy & 1,225,029  &  14, 951 \\
%GLDv2-noisy & 4,132,914  &  203,094 \\
GLDv2-clean & 1,580,470 & 81,313 \\ \midrule \rowcolor{LightCyan}
$\cR$GLDv2-clean (ours) &  1,578,905 & 81,296 \\
%ours-clean & 513,768 & 156,331 \\
%ours-clean$\ge15$ & 101,285 & 2,430 \\
\bottomrule
\end{tabular}
\vspace{-6pt}
\caption{Statistics of clean landmark training sets for image retrieval.}
\label{tab:table2}
\end{table}
%------------------------------------------------------------------------------

\paragraph{Revisited GLDv2-clean ($\cR$GLDv2-clean)}

By removing a number of landmark categories from GLDv2-clean as specified above, we derive a revisited version of the dataset, which we call \emph{$\cR$GLDv2-clean}. As shown in \autoref{tab:table1}, \rox and \rpa have landmark overlap with GLDv2-clean respectively for 36 and 38 out of 70 queries, which corresponds to a percentage of 51\% and 54\%, respectively. This is a very large percentage, as it represents more than half queries in both evaluation sets. In the new dataset, we remove 1,565 images from 18 GIDs of GLDv2-clean.

\autoref{tab:table2} compares statistics between existing clean datasets and the new $\cR$GLDv2-clean. We observe that a very small proportion of images and landmark categories are removed from GLDv2-clean to derive $\cR$GLDv2-clean. Yet, it remains to find what is the effect on retrieval performance, when evaluated on \rox and \rpa. For fair comparisons, we exclude from our experiments previous results obtained by training on GLDv2-clean; we limit to NC-clean, SfM-120k and the new $\cR$GLDv2-clean.


==> tex/sec_dataset-3.tex <==
\section{Revisiting Google Landmarks v2}
\label{sec:dataset}

%------------------------------------------------------------------------------
\begin{figure*}
\centering
\fig[1.0]{2}
\vspace{-20pt}
\caption{\emph{Confirming overlapping landmark categories} between training sets (GLDv2-Clean, NC-Clean, SfM-120k) and evaluation sets (Oxford5k, Paris6k). Green box (left): \roxf; blue box (right): \rpar. Top row: GLDv2-clean; middle row: NC-clean; bottom row: SfM-120k. Red box: query image. The query image from the evaluation set in each box/row is followed by top-5 most similar images from the training set. Pink box: training image landmark identical with query (evaluation) image landmark.
More examples can be found in the Appendix.
%(\autoref{fig:fig2_sup}).
\CH{I can't do this for each image. Top5 was generated by a randomized code as a result. Therefore, I generated 6 pdfs with one result each. (2\_*\_*.pdf)}
\iavr{Thanks, 6 pdf is still ok, but there are no pink boxes in the 6 pdf. I could add them myself in Latex if each image was separate, but I cannot do anything now. Can you create again with pink boxes? Can you also add a bit of space between images and a little more space between query and retrieved? As I said, PDFs are not needed here. They can be png/jpg.}
\CH{Look at the figure named "f2\_*\_*\_*.png".}
\iavr{Thanks, I will try. Is it possible to do at higher resolution? They are too small.}
}
\label{fig:fig2}
\end{figure*}
%------------------------------------------------------------------------------

\paragraph{Motivation}

A key weakness of current landmark retrieval datasets is their fragmented origins: training and evaluation sets are often independently collected and released by different studies. Initial datasets contained tens of thousands of images, a number that has now grown into the millions.

\emph{Evaluation sets} such as Oxford5k (\oxf5k)~\cite{Philbin01} and Paris6k (\paris6k)~\cite{Philbin02}, as well as their more recent versions, Revisited Oxford (\roxf~or \rox) and Paris (\rpar~or \rpa)~\cite{RITAC18}, are commonly used for benchmarking. Concurrently, \emph{training sets} such as \emph{Neural Codes} (NC)~\cite{Babenko01}, \emph{Neural Codes clean} (NC-clean)~\cite{Gordo01}, SfM-120k~\cite{Radenovic01}, Google Landmarks v1 (GLDv1)~\cite{delf}, and Google Landmarks v2 (GLDv2 and GLDv2-clean)~\cite{Weyand01} have been sequentially introduced and are widely used for representation learning.

These training sets are typically curated according to two criteria: first, to depict particular landmarks, and second, to not contain landmarks that overlap with those in the evaluation sets. They are originally collected by text-based web search using particular landmark names as queries. This often results in \emph{noisy} images in addition to images depicting the landmarks. Thus, NC, GLDv1 and GLDv2 are \emph{noisy} datasets. To solve this problem, images are filtered in different ways~\cite{Gordo01, Radenovi01} to ensure that they contain only the same landmark (instance). Accordingly, NC-clean, SfM-120k, and GLDv2-clean are \emph{clean} datasets.

The \emph{clean} datasets are also typically filtered to remove overlap with the evaluation sets. However, while NC-clean and SfM-120k adhere to both criteria, GLDv2-clean falls short of the second criterion. This discrepancy is not a limitation of GLDv2-clean per se, because the dataset comes with its own split of training, index and query images. However, the community is still using the \roxf and \rpar evaluation sets, whose landmarks have not been removed from GLDv2-clean. Besides, landmarks are still overlapping between the GLDv2-clean training and index sets.

This discrepancy is particularly concerning because GLDv2-clean is the most common training set in state-of-the-art studies. It has been acknowledged in previous work~\cite{superfeatures} and in broader community discussions\footnote{\url{https://github.com/MCC-WH/Token/issues/1}}. The effect is that results of training on GLDv2-clean are not directly comparable with those of training on NC-clean or SfM-120k. Results on GLDv2-clean may show artificially \emph{inflated performance}. This is often attributed to its larger scale but may in fact be due to overlap. Our study aims to address this problem by introducing a new version of GLDv2-clean.

%------------------------------------------------------------------------------

\paragraph{Identifying overlapping landmarks}

First, it is necessary to confirm whether common landmark categories exist between the training and evaluation sets. We extract image features from the training sets GLDv2-clean, NC-clean, and SfM-120k, as well as the evaluation sets \rox and \rpa. The features of the training sets are then indexed and the features of the evaluation sets \rox and \rpa are used as queries to search into the training sets.

\autoref{fig:fig2} displays the results. Interestingly, none of the retrieved images from NC-clean and SfM-120k training sets depict the same landmark as the query image from the evaluation set. By contrast, the top-5 most similar images from GLDv2-clean all depict the same landmark as the query. This suggests that using GLDv2-clean for training could lead to artificially \emph{inflated performance} during evaluation, when compared to NC-clean and SfM-120k. Since such comparison is unfair, the validity of previous studies that use GLDv2-clean for training should be reconsidered.

%------------------------------------------------------------------------------
\begin{figure}[t]
\centering
\fig[.95]{f3.pdf}
\vspace{-6pt}
\caption{\emph{Ranking and verification pipeline} to remove landmark categories from GLDv2-clean that overlap with those of the \rox and \rpa evaluation sets and obtain the revisited version, $\cR$GLDv2-clean.
\iavr{Please, NC-Clean $\to$ NC-clean and GLDV2-Clean $\to$ GLDv2-clean, everywhere. I am doing this in the text but I cannot do figures.} 
\CH{I fixed it to your request.}
\iavr{It is still ``GLDV2-Clean''. Can you please change to ``GLDv2-clean''. Or, let me work on it directly online.}
\CH{Oops. I'm sorry.  My mistake.  I fixed it.}
}
\label{fig:figa1}
\end{figure}
%------------------------------------------------------------------------------

\paragraph{Verification}

\iavr{I think I have a better understanding now. Please check again this paragraph. The problem remaining with your approach is that you did not get any visual matches for ``Invalides''. This raises concerns that we may have missed other overlaps. Can you share the images for the ``Invalides'' GID?}
\CH{You can check the answers in slack.}

\alert{Now, focusing on GLDv2-clean training set, we verify the overlapping landmarks. Each image in this set belongs to a landmark category and each category is identified by a GID and has a landmark name. We begin by visual matching.} In particular, we retrieve images for each query image from the evaluation set as above and we filter the top-$k$ ranked images by two verification steps.

First, we automatically verify that the same landmark is depicted by using robust spatial matching on correspondences obtained by local features and descriptors. Second, since automatic verification may fail, three human evaluators visually inspect all matches obtained in the first step. We only keep matches that are confirmed by at least one human evaluator. \alert{For every query from the evaluation set, we collect all confirmed visual matches from GLDv2-clean and we remove the entire landmark category of the GID that appears more frequently in this image collection}. \iavr{Is this correct now?} \CH{right.}

\alert{Independently, we collect all GIDs where the landmark name contains ``Oxford'' or ``Paris'' and we also mark them as candidate for removal. The entire landmark category of a GID is removed if it is confirmed by at least one human evaluator that it is in one the evaluation sets. This is the case for ``Hotel des Invalides Paris''. \autoref{fig:figa1} illustrates the complete ranking and verification process.} \iavr{Is this correct?} \CH{right.}

%------------------------------------------------------------------------------
\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{3.2pt}
\begin{tabular}{lcccc} \toprule
\Th{Eval} & \Th{\#Eval Img} & \Th{\#Dupl Eval} & \Th{\#Dupl GLDv2 GID} & \Th{\#Dupl GLDv2 Img} \\\midrule
\rox & 70 & 36 (51\%) &  10 & 1227 \\
\rpa & 70 & 38 (54\%) &   7 & 315 \\
Text &  &  &  1  & 23 \\ \midrule
Total & 140 & 74  & 18 & 1565 \\
\bottomrule
\end{tabular}
\vspace{-6pt}
\caption{Statistics of GLDv2-clean training images / landmark categories that overlap (are duplicate) with \rox and \rpa evaluation sets and are removed in our $\cR$GLDv2-clean. \Th{Eval}: evaluation sets; \Th{Dupl}: duplicated; \Th{GID}: GLDv2 category; \Th{Img}: image. \iavr{We need to provide the names of GIDs in the Appendix.} \CH{GIDs: 6190, 19172, 28949, 37135, 42489, 44923, 47378, 69195, 138332, 144472, 145268, 146388, 147275, 152496, 167104, 167275, 181291, 192090 - I will double-check before submission.} \iavr{But, each GID also has a landmark name, right? Then, for each one of the 18 removed classes, report GID (number), landmark name from GLDv2-clean, landmark name from Oxford/Paris and which test set it overlaps (Oxford or Paris). That's a table with 4 columns, to be added in the Appendix. Can you do that?} \CH{I'll let you know when I finalize this.} \CH{I created a new Table.A10 and completed it.}}
\label{tab:table1}
\end{table}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}
\centering
\scriptsize
% \setlength{\tabcolsep}{15.5pt}
\begin{tabular}{lcc} \toprule
\Th{Training Set} & \Th{\#Images} & \Th{\#Categories} \\ \midrule
%NC-noisy & 213,678 & 672 \\
NC-clean & 27,965 & 581 \\
SfM-120k & 117,369 & 713 \\
%GLDv1-noisy & 1,225,029  &  14, 951 \\
%GLDv2-noisy & 4,132,914  &  203,094 \\
GLDv2-clean & 1,580,470 & 81,313 \\ \midrule \rowcolor{LightCyan}
$\cR$GLDv2-clean (ours) &  1,578,905 & 81,296 \\
%ours-clean & 513,768 & 156,331 \\
%ours-clean$\ge15$ & 101,285 & 2,430 \\
\bottomrule
\end{tabular}
\vspace{-6pt}
\caption{Statistics of clean landmark training sets for image retrieval.}
\label{tab:table2}
\end{table}
%------------------------------------------------------------------------------

\paragraph{Revisited GLDv2-clean ($\cR$GLDv2-clean)}

By removing a number of landmark categories from GLDv2-clean as specified above, we derive a revisited version of the dataset, which we call \emph{$\cR$GLDv2-clean}. As shown in \autoref{tab:table1}, \rox and \rpa have landmark overlap with GLDv2-clean respectively for 36 and 38 out of 70 queries, which corresponds to a percentage of 51\% and 54\%, respectively. This is a very large percentage, as it represents more than half queries in both evaluation sets. In the new dataset, we remove 1,565 images from 18 GIDs of GLDv2-clean.

\autoref{tab:table2} compares statistics between existing clean datasets and the new $\cR$GLDv2-clean. We observe that a very small proportion of images and landmark categories are removed from GLDv2-clean to derive $\cR$GLDv2-clean. Yet, it remains to find what is the effect on retrieval performance, when evaluated on \rox and \rpa. For fair comparisons, we exclude from our experiments previous results obtained by training on GLDv2-clean; we limit to NC-clean, SfM-120k and the new $\cR$GLDv2-clean.


==> tex/sec_exp_abl-1.tex <==
\subsection{Ablation study}

Beyond the core experimental results discussed here, ~\autoref{sec:mAblation} delves into more extensive and detailed ablation studies.

% 먼저, 이번장의 실험결과 이외에 ~\autoref{sec:mAblation}에 더 다양하고 상세한 Ablation Study 에 대한 실험 결과들이 있음을 알린다.

\paragraph{Design ablation}

\autoref{sec:1-stage} evaluates the impact of each component on the overall performance of the proposed model. The ablation study proceeds in the following order: Base (Backbone), Selective Context Module (SCM), AL, and Enhanced Backbone Module (EBM).
\CH{As an initial correction, there is no mention of SCM, EBM at all in the text.} \iavr{I know, that's why I asked you to write something here. I repeat my comment: ``The idea is that instead of designing components specifically for retrieval, we explore existing ideas for "enhancing the backbone" and for "representing context" (or the names that you prefer), which are benchmarked in the appendix and the best (EBM, SCM) are employed in table 7.''} 
\CH{I've added these directly below. 
Please let me know if this is not what you intended.}
\alert{Our network consists of the four modules mentioned above.}
Here, Base signifies a model where only GeM is applied to the ResNet101 backbone.
%
\alert{SCM is inspired by previous work~\cite{Chen2017RethinkingAC, sknet} and proposes a way to enrich spatial and contextual information to apply locality more effectively.
}
\alert{EBM is intended to enhance the performance of the CNN backbone. 
To do this, we apply previous studies~\cite{Hu01, wang01, Wang02, GatherExcite} in a \emph{plug and play} manner. }
\alert{AL has already been described in \autoref{sec:1-stage} as our main algorithm.
}
%
\autoref{tab:components} provides a comparative analysis of each experiment, illustrating performance gains achieved with the incremental inclusion of proposed modules.

% % 우리가 제안한 구조에서 각 구성 요소가 모델 성능에 미치는 영향들을 평가한다.
% \autoref{sec:1-stage}에서 언급한 각 구성 요소가 우리가 제안한 모델에 미치는 영향을 평가한다. Base, SCM, ALM, EBM의 순으로 ablation study를 진행한다. 
% Base는 ResNet101 Backbone에 대하여 GeM만을 적용시킨 방법을 의미한다.
% \autoref{tab:components}에서 각 실험 결과를 볼 수 있고, 우리가 제안한 모듈이 추가될때마다 성능이 향상되었음을 보여준다.

%------------------------------------------------------------------------------
\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{3.0pt}
\begin{tabular}{l*{11}{c}} \toprule
& \mr{2}{Base}  & \mr{2}{SCM} & \mr{2}{AL} & \mr{2}{EBM} & \mr{2}{\Th{Oxf5k}} & \mr{2}{\Th{Par6k}} & \mc{2}{\Th{Medium}} & \mc{2}{\Th{Hard}} \\ \cmidrule(l){8-11}
&&     & & & &  & \rox & \rpa & \rox & \rpa  \\ \midrule
%
& \ch    &     &     &      &   80.2    & 83.2       & 55.1       & 67.7     & 25.8      & 40.7 \\
& \ch    & \ch &     &      &   87.6    & 90.7       & 64.7       & 76.6      & 38.2      & 52.7 \\
& \ch    & \ch & \ch &      &   89.7    & \tb{92.0}  & 67.0       & \tb{79.4} & 41.0      & 57.4 \\
& \ch    & \ch & \ch & \ch  & \tb{89.9} & \tb{92.0} & \tb{67.3} & \tb{79.4} & \tb{42.4} & \tb{57.5} \\ 
\bottomrule
\end{tabular}
\vspace{-6pt}
\caption{mAP comparison of variants of our modules with/without different components. Training on SfM-120k.
\CH{\\ Since I modified it to exclude only ALM, it was moved from the main text to Appendix. There is no mention of SCM, EBM in the text at all. So shouldn't this table be moved to Appendix as well?}
\iavr{\\ No no no. It should stay here. First, ALM is a main contribution, we need to know its contribution. Next, SCM, EBM are used our best results reported in other tables. So we need to know their contibution too. I asked to you write something about SCM, EBM in the text. The ablation of SCM alternatives (Table A11) and EBM alternatives (Table A10) remains in the appendix.}
\CH{\\ And, "EBM - SCM - ALM" is correct, that's what we did at first. The check order didn't work out that way, so we ended up with the current situation. (If it makes sense to change it, feel free to fix it). BTW, the implementation order is actually EBM was added last.}
\iavr{\\ I now realize that, to change the order, you need to redo experiments. In this sense, leave it for later. EBM - SCM - ALM looks like a more natural order, as it is the order of computation. But in fact, you could do all (8) combinations (when you have time).}
\CH{\\ SCM is a combination of "multi-scale spatial context Information" (formula (A6)) + ACI, as shown in the original main figure (see 3.png). I think we can just combine them if there is a problem.}
\iavr{\\ Formula (A6) is EBM; you must mean (A7). Then again, ACI~\cite{sknet} does include dilated convolutions followed by BN and ReLU, similarly to (A7). Your figure of SCM is almost the same as fig. 1 of ACI. The only difference I see is several dilated convolutions combined with weights in (A8), while ACI has only two that are summed without weights. From what I see, it is safer, at least for now, to just say that SCM is ACI. Am I missing something?}
\CH{You're right. 
I just separated them and modified them a bit differently to make them look as different as possible. With this change, the performance is slightly higher than ASPP and SKNet. }
}

\label{tab:components}
\end{table}
%------------------------------------------------------------------------------

\paragraph{Binary map background value}

This experiment focuses on constructing the Binary Map $\vB$ within the ALM described in \autoref{sec:1-stage}. Instead of assigning a fixed value of 0 to the background and 1 to the object, we propose variability to the background value using a random noise method, represented as $\epsilon$ in \autoref{eq:mask}. \autoref{tab:bgvalue} indicates that our method exhibits superior performance.

% \autoref{sec:1-stage}에서 설명한 ALM의 과정에서의 Binary Map $\vB$ 구성에 대한 실험이다. 
% 이 실험에서 단순히 background를 0, object를 1로 fixed value로 주는 것보다, 우리는 background value 를 Random Noise 방법 (\autoref{eq:mask}의 $\epsilon$)으로 주는 방법을 제안한다.
% \autoref{tab:bgvalue}는 이에 대한 실험결과를 보여주며, 이 결과에서 우리가 제안한 방법이 더 좋은 성능을 보여준다.

%------------------------------------------------------------------------------
\begin{table}
\centering
\small
%\tiny
\setlength{\tabcolsep}{2.0pt}
\begin{tabular}{l*{7}{c}} \toprule
\mr{2}{\Th{Value}} & \mr{2}{\Th{Oxf5k}} & \mr{2}{\Th{Par6k}} & \mc{2}{\Th{Medium}} & \mc{2}{\Th{Hard}} \\ \cmidrule(l){4-7}
 & & &  \rox & \rpa & \rox & \rpa \\ \midrule
Scalar (0) & 87.4 & 91.6 & 64.9  & 77.5 & 39.1 & 53.8  \\
Scalar (0.5) & 87.5 & 91.7 & 64.8 & 77.7 & 38.8 & 54.3  \\
$\mathcal{N}$ (0.1, 0.5) & 90.2 & 90.5 & 67.4 & 78.1 & 40.2 & 55.2  \\
% $\mathcal{N}$(0.1, 0.7) & 89.4 & 91.7 & 66.4 & 78.2 & 39.7 & 55.1  \\
$\mathcal{N}$ (0.1, 0.9) (Ours) & \tb{89.9} & \tb{92.0} & \tb{{67.3}}&  {\tb{79.4}}& {\tb{42.4}} & {\tb{57.5}}\\ \bottomrule
\end{tabular}
\vspace{-6pt}
\caption{mAP comparison of \emph{Binary Map's background value} in our model. Training on SfM-120k.}
\label{tab:bgvalue}
\end{table}
%------------------------------------------------------------------------------

\paragraph{Thresholds for binary map construction}

This experiment further explores the construction of the binary map $\vB$, as defined in \autoref{eq:mask}, within the ALM framework described in \autoref{sec:1-stage}. The binary map is constructed by the spatial attention map $\vF^{s}$ from \autoref{eq:attn}. We experiment with varying predefined threshold values for this attention map, which ranges between 0 and 1. \autoref{tab:thresholds} shows that optimal performance is achieved when the threshold is set to 2.

% \autoref{sec:1-stage}에서 설명한 ALM의 과정에서의 \autoref{eq:mask}의 Binary Map $\vB$ 구성에 대한 실험이다.
% 이때 $\vB$는 \autoref{eq:attn}의 spatial attention map $\vF^{s}$에 의해 구성된다. 
% spatial attention map은 0 $\sim$ 1사이 값을 가지고 있기 때문에, 미리 정의된 threshold값들에 의해 다르게 재구성된다. 
% \autoref{tab:thresholds}는 이에 대한 결과를 보여준다. 
% threshold가 2개로 구성될때 가장 좋은 결과를 보여준다.

%------------------------------------------------------------------------------
\begin{table}
\centering
\small
%\tiny
\setlength{\tabcolsep}{3.0pt}
\begin{tabular}{l*{7}{c}} \toprule
\mr{2}{\Th{\#Threshold}} & \mr{2}{\Th{Oxf5k}} & \mr{2}{\Th{Par6k}} & \mc{2}{\Th{Medium}} & \mc{2}{\Th{Hard}} \\ \cmidrule(l){4-7}
 & & &  \rox & \rpa & \rox & \rpa \\ \midrule
6 & 89.4 & 91.6 & 66.5  & 78.1 & 40.5 & 55.0  \\
3 & 89.4 & \tb{92.2} & \tb{67.5} & 78.5 & \tb{42.4} & 55.3  \\
2 (Ours) & \tb{89.9} & {92.0} & {{67.3}}&  {\tb{79.4}}& {\tb{42.4}} & {\tb{57.5}} &
\\
1 & {87.5} & {91.7} & {64.8}&  {77.7}& {38.8} & {54.3}\\ \bottomrule
\end{tabular}
\vspace{-6pt}
\caption{mAP comparison of \Th{\#thresholds} for \emph{Binary Map Construction} in our model. Training on SfM-120k.
\CH{The number of "multiple threshols" in fig.4 refers to the number of thresholds. The \#Threshold =1 case was missing, so I added it.}
\iavr{This is great!}
}
\label{tab:thresholds}
\end{table}
%------------------------------------------------------------------------------


==> tex/sec_exp_bench-1.tex <==
%------------------------------------------------------------------------------
\begin{table*}
\input{exp/clean_datasets}
\vspace{-6pt}
\caption{mAP comparison of SOTA using \emph{Clean-DataSets}. AF:ArcFace loss. 
TP:Triplet loss. CLS:Softmax Loss. SIA:Siamese loss. SOS:Second-Order Similarity Loss. MSE: Mean Squared Loss. R101/R50: ResNet101/50. V16: VGG16. A:AlexNet. [O]: Off-the-shelf (pre-trained on ImageNet). \Th{SelfLoc}:Self Localization (Unsupervised-Learning). GAP:Global Average Pooling. GSP:Global Sum Pooling. 
\Th{E2E}:End-to-End. \Th{FT}:Fine-Tuned. Black bold: best previous methods in block. Red: best results. Blue: Ours results higher than previous methods. SP: spatial verification.  $^*$: $d=256$~\cite{Babenko03}. --:Not present or unconfirmed. }
%$\dagger/\ddagger$: training using official/our code. }
\label{tab:sota_cleandata}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\input{exp/1m}
\vspace{-6pt}
\caption{
%mAP comparison of our model against SOTA methods and different training sets.
mAP comparison by Previous \vs Ours.   
Red: best results. Black bold: best previous methods. Blue: Ours results higher than previous methods.
A: AlexNet; V16: VGG16; R50/101:Resnet50/101.
\Th{FT}:fine-tuning. $\dagger$: reproduced. 
}
\label{tab:1m}
\end{table*}
%------------------------------------------------------------------------------

\subsection{Benchmark}
\label{sec:exp-bench}

\paragraph{Detect-to-Retrieve ($\mathbf{D2R}$)}

\autoref{tab:sota_cleandata} offers a comparative assessment of various $\mathbf{D2R}$ methodologies. 
%, excluding those that employ \Th{Global Descriptors+Revisiting GLDV2}. 
Remarkably, the method proposed in this study outperforms the highest-ranking approach by Liao et al.~\etal~\cite{Liao01}, which was trained on the SfM-120k dataset. Specifically, our method improves performance by 12.5\% on the \oxf5k dataset and by 4.8\% on the \paris6k dataset.
% \autoref{tab:sota_cleandata}에서 $\mathbf{D2R}$ 연구들을 비교 (\Th{Global Descriptors+Revisiting GLDV2} 연구 제외) 해볼때, SfM-120k로 학습한 연구 중 가장 높은 성능을 보인 Liao~\etal~\cite{Liao01}보다 우리의 연구가 각각 \oxf5k, \paris6k Base에서 12.5\%, 4.8\%가 향상된 것을 보여준다
% % \autoref{tab:sota_cleandata}에서 이전 $\mathbf{D2R}$ 연구와 비교 (\Th{Global Descriptors+Revisiting GLDV2} 연구 제외) 해볼때, 이전 연구에서 가장 좋은 Liao~\etal~\cite{Liao01}에서, 우리의 SfM-120k로 학습한 연구가  각각 \oxf5k, \paris6k Base에서 12.5\%, 4.8\%가 향상된 결과를 보여주었다. 
% . 
%
% %\autoref{tab:sota_cleandata}에서 \Th{FINETUNED} 항목은 바로 ImageNet pre-trained model를 이용했다는 것이 아니라, 한번더 학습셋으로 학습한 후, 이 학습한 모델을 이용하여 fine-tuning에 적용했다는 의미이다. 
% %본 연구는 이 단계를 걷치지 않고도 더 좋은 성능을 달성하였다.
% %특히, \autoref{tab:1m}에서 이를 적용한 방법과 1 million distractors (\r 1m)에 적용에 대한 보다 상세한 실험 결과를 볼 수 있다.
In \autoref{tab:sota_cleandata}, the categories of \emph{E2E} and \emph{SelfLoc} are exclusive to studies in the \emph{Global Descriptors+$\mathbf{D2R}$} section. \emph{E2E} refers to end-to-end learning in a single-stage pipeline, whereas \emph{SelfLoc} represents unsupervised learning methods that do not require location information. Interestingly, studies in this category employ different training sets, as no single dataset provides annotations for both $\mathbf{D2R}$ tasks. Our study is unique in meeting both \emph{E2E} and \emph{SelfLoc} criteria, thereby eliminating the need for a detection-related training set.
% \autoref{tab:sota_cleandata}에서 \emph{E2E}와 \emph{SelfLoc} 항목은 \emph{Global Descriptors+Detected to Retrieval}에만 존재하는 항목이다.
% \emph{E2E}는 End-to-End 학습의 Single-Stage Pipeline 방법을 의미하고, Localization은 위치 정보가 필요한데 이를 필요치 않는 Unsupervised Learning방법을 \emph{SelfLoc}라 한다. 
% \emph{Global Descriptors+Detected to Retrieval} 연구들의 \emph{TrainSet} 항목을 보면, 다양한 학습셋을 적용했는데, 이는 Detection과 Retrieval이 동시에 annotation된 데이터셋이 없기 때문이다.
% 결과적으로, 우리는 Detection관련 학습셋이 필요없는 \emph{E2E}과 \emph{SelfLoc}조건에 맞는 유일한 연구라할 수 있다.

%------------------------------------------------------------------------------

\paragraph{Existing clean dasasets: \emph{NC-clean, SfM-120k}}

In this context, clean datasets refer to NC-clean and SfM-120k. \autoref{tab:sota_cleandata} also presents a performance comparison.
%, excluding studies that \Th{Global Descriptors+Revisiting GLDV2}. 
While some existing works~\cite{Gordo01, delf} leverage classification models for fine-tuning (marked as \tb{Y} in the table), our research (\autoref{fig:A5_FT}) explores both fine-tuned and non-fine-tuned approaches. We demonstrate SOTA performance across all evaluations. In terms of comparison, our method shows notable improvements over AGeM~\cite{gu2018attention}, which was previously considered the best approach.
We improve by 2.9\%, 0.6\% on \oxf5k, \paris6k Base, 9.2\%, 18.2\% on \rox, \rpa Medium, and 6.4\%, 9.5\% on \rox, \rpa  Hard. Further details, including results with a 1M distractor, are available in \autoref{tab:1m}.
%
% 여기서 Clean Dasetset은 NC-clean, SfM-120k 데이터셋을 의미한다. 
% \autoref{tab:sota_cleandata}은 이에 대한 성능 비교 (\Th{Global Descriptors+Revisiting GLDV2} 연구 제외)를 보여준다. 
% 몇몇 연구~\cite{Gordo01, delf}들은 분류 기반으로 학습한 모델을 fine-tuning에 적용하였고, 테이블에서 \emph{Fine-Tuned}의 \tb{Y} 로 표시된 경우가 이에 해당한다.
% 우리는 fine-tuning을 적용한것과 적용하지 않은 방법에 대해 모두 보여준다. 
% % 우리는 2가지 방법의 결과를 보여주고 있는데, 몇몇 이전 연구~\cite{Gordo01, delf}들은 분류 기반으로 학습한 후, 다시 이 학습한 모델을 이용하여 다시 fine-tuning에 적용한 경우가 있었는데, 이 테이블에서 \emph{Fine-Tuned}의 \tb{Y} 로 표시된 경우가 이에 해당한다.
% %이 테이블 결과에서 우리는 \Th{Paris6k} 항목을 제외한 모든 평가 항목에서 SOTA 성능을 보여주었다. 
% 이 결과에서 우리는 모든 평가 항목에서 SOTA 성능을 보여주었다. 
% %이전 연구에서 AGeM~\cite{gu2018attention}이 가장 좋은 결과를 보여주고 있는데, 각각 \rox, \rpa Medium 에서, 0.3\%, 1.3\%, \rox, \rpa Hard 에서 1.7\%, 0.2\% 가 향상된 결과를 보였다. 
% GD를 이용한 이전 연구에서 AGeM~\cite{gu2018attention}이 가장 좋은 결과를 보여주고 있는데, 우리 결과와 비교해 볼때, we improve by 2.9\%, 0.6\% on \oxf5k, \paris6k Base and 9.2\%, 18.2\% on \rox, \rpa Medium and by 6.4\%, 9.5\% on \rox, \rpa Hard.
% %또한, 이전 $\mathbf{D2R}$ 연구와 비교해볼때도, 이전 연구에서 가장 좋은 Liao~\etal~\cite{Liao01}에서, 우리의 연구가 각각 \oxf5k, \paris6k Base에서 9.8\%, 1.7\%가 향상된 결과를 보여주었다. 
% 덧붙여, \autoref{tab:1m}에서 1M distractor를 포함한 보다 상세한 항목에 대한 평가 결과를 볼 수 있다.
%

%------------------------------------------------------------------------------

\paragraph{New clean dataset: \emph{$\cR$GLDV2-clean}}

\autoref{sec:dataset} describes \emph{$\cR$GLDV2-clean}, a new dataset developed for this study. The results of applying the new data are shown in \autoref{tab:1m}. We also presents full experimental results, including the impact of introducing 1 million distractors (\r 1m) into the dataset. Although we attempted to reproduce previous SOTA algorithms, complete replication for all previous experiments, proved challenging. This is largely because \emph{$\cR$GLDV2-clean} requires a large amount of data (approximately 15 million), and many previous SOTA methods have not publicly disclosed their source codes. To ensure a fair evaluation, our experiments employed the same ResNet101 backbone~\cite{Gordo01, Kalantidis01, Radenovic01, gu2018attention, Ng01, Yokoo01, SCH01, yang2021dolg, tokens} and ArcFace loss~\cite{Yokoo01, SCH01, yang2021dolg, tokens, dtop} used in previous studies. Wherever possible, we used publicly available official codes. It is also worth noting that previous comparative evaluations often employed different training sets while using the same evaluation set, which could introduce bias. Our study, however, utilizes the same training and evaluation sets to ensure fairness. 
% Some metrics under $\mathbf{S_{2}D2R}$ in {\rpa+\r1m} underperform, but 
$\mathbf{S_{2}D2R}$+$\Th{FT}$ consistently outperforms across most evaluation criteria. When comparing our $\mathbf{S_{2}D2R}$ outcomes to previous studies, we achieve a 5.1\% improvement on \rox$+$\r1m~(medium) and a 2.5\% improvement on \rox$+$\r1m~(hard), excluding \rpar on \r1m. With fine-tuning ($\mathbf{S_{2}D2R}$+$\Th{FT}$), our model establishes new SOTA results for nearly all tested metrics. In other words, we improve by 10.2\%, 5.5\% on \rox, \rpar$+$\r1m~(medium) and by 16.9\%, 2.1\% on \rox, \rpar$+$\r1m~(hard). The results affirm that our method surpasses previous studies.
%
% \autoref{sec:dataset} describes \emph{$\cR$GLDV2-clean}, a new dataset developed for this study. The results of applying the new data are shown in \Th{Global Descriptors+Revisiting GLDV2} in \autoref{tab:1m}. Although we attempted to reproduce previous SOTA algorithms, complete replication for all previous experiments, proved challenging. This is largely because \emph{$\cR$GLDV2-clean} requires a large amount of data (approximately 15 million), and many previous SOTA methods have not publicly disclosed their source codes. To ensure a fair evaluation, our experiments employed the same ResNet101 backbone~\cite{Gordo01, Kalantidis01, Radenovic01, gu2018attention, Ng01, Yokoo01, SCH01, yang2021dolg, tokens} and ArcFace loss~\cite{Yokoo01, SCH01, yang2021dolg, tokens, dtop} used in previous studies. Wherever possible, we used publicly available official codes. It is also worth noting that previous comparative evaluations often employed different training sets while using the same evaluation set, which could introduce bias. Our study, however, utilizes the same training and evaluation sets to ensure fairness. The results affirm that our method surpasses previous studies.
% 우리는 \autoref{sec:dataset}에서 우리의 새로운 데이터셋인 \emph{$\cR$GLDV2-clean}에 대한 설명을 하였다.
% \autoref{tab:sota_cleandata}의 \Th{Global Descriptors+Revisiting GLDV2}에서 새로운 데이터를 적용한 결과를 볼 수 있다.
% 우리는 이 실험을 위해서, 이전 SOTA 알고리즘을 리프로듀싱하였지만 이전의 모든 실험에 대해 완벽히 리프로듀싱하기는 어려움이 있다. 
% \autoref{tab:table2}에서 보듯이, \emph{$\cR$GLDV2-clean}는 약 15M장의 많은 데이터, 각각의 학습에 적용 된 다양한 Sampling 방식, 그리고 이전의 많은 SOTA 방법의 소스들 공개되지 않은 점 때문이다.
% %특히, 장비의 제약이 있었다. 학습에 이용한 장비는 \autoref{sec:Implementation}에서 확인할 수 있다. 
% % 특히, \autoref{sec:Implementation}에서 언급한 장비로는 제약이 있었다.
% 우리는 이러한 제약조건에서, 최대한 공정한 실험을 위해, 기존 연구들에서 가장 많이 적용된, Resnet101 backbone~\cite{Gordo01, Kalantidis01, Radenovic01, gu2018attention, Ng01, Yokoo01, SCH01, yang2021dolg, tokens}과 ArcFace loss~\cite{Yokoo01, SCH01, yang2021dolg, tokens, dtop}를 고정시켜 각 이전 연구에 적용되었던 네트워크들과 함께 \emph{$\cR$GLDV2-clean} 데이터셋를 적용시켜 실험한다. 
% 그리고 이전 연구에 적용되었던 네트워크들은 최대한 공개된 official code를 이용하였다.
% 또한, 이전 연구들의 비교 평가는 평가셋은 동일하지만, 다른 학습셋을 적용한 연구들과 비교한 경우들이다. 
% 이 점은 불공평한 평가 결과를 제공한다고 생각한다.
% 우리는 공평한 평가를 위해 학습셋과 평가셋을 동일하게 하여 실험하였다.
% %\autoref{tab:sota_cleandata}는 이에 대한 우리의 실험 결과를 보여준다.
% %이 실험 결과에서 우리가 제안한 방법이 이전 연구보다 더 뛰어난 성능을 보여주고 있다.
% 실험 결과에서 우리가 제안한 방법이 이전 연구보다 더 뛰어난 성능을 보여주고 있다.


==> tex/sec_exp_bench-2.tex <==
%------------------------------------------------------------------------------
\begin{table*}
\input{exp/clean_datasets}
\vspace{-6pt}
\caption{mAP comparison of SOTA on \emph{clean} training sets (no overlap with evaluation sets).
\Th{FT}: fine-tuning; \Th{E2E} ($\mathbf{D2R}$ only): end-to-end training; \Th{Loc} ($\mathbf{D2R}$ only): localization supervision. 
\emph{Network}: R50/101: ResNet50/101; V16: VGG16; A: AlexNet. 
\emph{Pooling}: GAP: global average pooling; GSP: global sum pooling.
\emph{Loss}: AF: ArcFace; TP: triplet; CLS: softmax; SIA: siamese; SOS: second-order similarity; MSE: mean square errorl; LOCAL: Localization Loss;
SP: spatial verification.
[O]: Off-the-shelf (pre-trained on ImageNet).
Red: best result; blue: our results higher than previous methods; black bold: best previous method per block.
\iavr{References are wrong, please check. What do we mean by fine-tuning? Aren't all methods fine-tuning? We should report separately the training set for detection and for retrieval, if applicable (in two separate columns).}
\CH{This reference seems to be correct. 
The results on the actual training set are from a different study, so the reference looks different.
I will check again tomorrow.}
\CH{Can we say that ASMK, the aggregated method of LD, is a pooling method? It's ambiguous. }
% $^*$: $d=256$~\cite{Babenko03}. --: Not present or unconfirmed. 
%$\dagger/\ddagger$: training using official/our code.
}
\label{tab:sota_cleandata}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\input{exp/1m}
\vspace{-6pt}
\caption{Comparison of SOTA on the new ($\cR$GLDv2-clean) as well as existing (SfM-120k) clean traing set (no overlap with evaluation sets). Red: best results; blue: our results higher than previous methods; black bold: best previous method per block.
% A: AlexNet; V16: VGG16; R50/101:Resnet50/101.
\Th{FT}:fine-tuning. \alert{†/‡: official/our code.} \iavr{Please indicate separately, which methods use official code and which not.}
}
\label{tab:1m}
\end{table*}
%------------------------------------------------------------------------------

\subsection{Comparison with state of the art}
\label{sec:exp-bench}

\paragraph{Existing clean datasets}

\autoref{tab:sota_cleandata} provides a comparative assessment of different methods based on global or local descriptors, with or without a $\mathbf{D2R}$ approach, on existing \emph{clean datasets}, referring to training sets that do not overlap with the evaluation sets, in particular to NC-clean and SfM-120k. \alert{While some existing works~\cite{Gordo01, delf} leverage classification models for fine-tuning, our work (\autoref{fig:A5_FT}) explores both fine-tuned and non-fine-tuned approaches. We refer to our method as $\mathbf{S_{2}D2R}$ without fine-tuning and $\mathbf{S_{2}D2R}$+$\Th{FT}$ with fine-tuning.} \iavr{What do we mean by fine-tuning? Aren't all methods using fine-tuning? Do you mean, learn our ALM on top of a frozen model, as pretrained on ImageNet, \vs fine-tuning \eg on SfM-120k? Like we compare in figures 5 and 7?}
\CH{FT: Same way as DIR, DELF. It means that the model generated as a result of classification training with landmark set(sfm120k, RGLDv2-clean) is used again to learn. However, the difference between DIR and DELF is that the existing R101 backbone freezes when training. Figure A11/A12 illustrates this. Should we say 2 stage fine-tuning?}
\iavr{I thought it was clear but now I am not sure again. Your definition of FT is essentially fig A10, where in the second stage of FT (b), the backbone is frozen. Both DIR and DELF have ``Y'' in FT column of table. But here you are saying that in addition, the backbone is \textbf{not} frozen for both DIR and DELF? For which one is it frozen and for which not?}

Comparing with methods using global descriptors without $\mathbf{D2R}$, our method demonstrates SOTA performance and brings significant improvements over AGeM~\cite{gu2018attention}, the previous best competitor. In particular, 2.9\%, 0.6\% mAP on \oxf5k, \paris6k Base, 9.2\%, 18.2\% on \rox, \rpa Medium, and 6.4\%, 9.5\% on \rox, \rpa Hard.
% Further details, including results with a 1M distractor, are available in \autoref{tab:1m}.
%
% 여기서 Clean Dasetset은 NC-clean, SfM-120k 데이터셋을 의미한다. 
% \autoref{tab:sota_cleandata}은 이에 대한 성능 비교 (\Th{Global Descriptors+Revisiting GLDV2} 연구 제외)를 보여준다. 
% 몇몇 연구~\cite{Gordo01, delf}들은 분류 기반으로 학습한 모델을 fine-tuning에 적용하였고, 테이블에서 \emph{Fine-Tuned}의 \tb{Y} 로 표시된 경우가 이에 해당한다.
% 우리는 fine-tuning을 적용한것과 적용하지 않은 방법에 대해 모두 보여준다. 
% % 우리는 2가지 방법의 결과를 보여주고 있는데, 몇몇 이전 연구~\cite{Gordo01, delf}들은 분류 기반으로 학습한 후, 다시 이 학습한 모델을 이용하여 다시 fine-tuning에 적용한 경우가 있었는데, 이 테이블에서 \emph{Fine-Tuned}의 \tb{Y} 로 표시된 경우가 이에 해당한다.
% %이 테이블 결과에서 우리는 \Th{Paris6k} 항목을 제외한 모든 평가 항목에서 SOTA 성능을 보여주었다. 
% 이 결과에서 우리는 모든 평가 항목에서 SOTA 성능을 보여주었다. 
% %이전 연구에서 AGeM~\cite{gu2018attention}이 가장 좋은 결과를 보여주고 있는데, 각각 \rox, \rpa Medium 에서, 0.3\%, 1.3\%, \rox, \rpa Hard 에서 1.7\%, 0.2\% 가 향상된 결과를 보였다. 
% GD를 이용한 이전 연구에서 AGeM~\cite{gu2018attention}이 가장 좋은 결과를 보여주고 있는데, 우리 결과와 비교해 볼때, we improve by 2.9\%, 0.6\% on \oxf5k, \paris6k Base and 9.2\%, 18.2\% on \rox, \rpa Medium and by 6.4\%, 9.5\% on \rox, \rpa Hard.
% %또한, 이전 $\mathbf{D2R}$ 연구와 비교해볼때도, 이전 연구에서 가장 좋은 Liao~\etal~\cite{Liao01}에서, 우리의 연구가 각각 \oxf5k, \paris6k Base에서 9.8\%, 1.7\%가 향상된 결과를 보여주었다. 
% 덧붙여, \autoref{tab:1m}에서 1M distractor를 포함한 보다 상세한 항목에 대한 평가 결과를 볼 수 있다.

%------------------------------------------------------------------------------

% \paragraph{Detect-to-Retrieve ($\mathbf{D2R}$)}

%, excluding those that employ \Th{Global Descriptors+Revisiting GLDV2}. 
\alert{Comparing with methods using global descriptors without $\mathbf{D2R}$, our method outperforms the highest-ranking approach by DIR+RPN~\cite{Gordo01}, which was trained on the SfM-120k dataset. Specifically, our method improves mAP by 7.4\% on \oxf5k dataset and by 1.1\% on \paris6k.} 
\iavr{But, Liao~\etal is not the best competitor. Can you please update?}
\CH{I added it later, so I'm a little late with the update.  I fixed it.}
% \autoref{tab:sota_cleandata}에서 $\mathbf{D2R}$ 연구들을 비교 (\Th{Global Descriptors+Revisiting GLDV2} 연구 제외) 해볼때, SfM-120k로 학습한 연구 중 가장 높은 성능을 보인 Liao~\etal~\cite{Liao01}보다 우리의 연구가 각각 \oxf5k, \paris6k Base에서 12.5\%, 4.8\%가 향상된 것을 보여준다
% % \autoref{tab:sota_cleandata}에서 이전 $\mathbf{D2R}$ 연구와 비교 (\Th{Global Descriptors+Revisiting GLDV2} 연구 제외) 해볼때, 이전 연구에서 가장 좋은 Liao~\etal~\cite{Liao01}에서, 우리의 SfM-120k로 학습한 연구가  각각 \oxf5k, \paris6k Base에서 12.5\%, 4.8\%가 향상된 결과를 보여주었다. 
% . 
%
% %\autoref{tab:sota_cleandata}에서 \Th{FINETUNED} 항목은 바로 ImageNet pre-trained model를 이용했다는 것이 아니라, 한번더 학습셋으로 학습한 후, 이 학습한 모델을 이용하여 fine-tuning에 적용했다는 의미이다. 
% %본 연구는 이 단계를 걷치지 않고도 더 좋은 성능을 달성하였다.
% %특히, \autoref{tab:1m}에서 이를 적용한 방법과 1 million distractors (\r 1m)에 적용에 대한 보다 상세한 실험 결과를 볼 수 있다.
Interestingly, methods in the $\mathbf{D2R}$ category employ different training sets, as no single dataset provides annotations for both $\mathbf{D2R}$ tasks. Our study is unique in being single-stage, end-to-end (\textsc{E2E}) trainable and at the same time requiring no localization supervision (\textsc{Loc}), thereby eliminating the need for a detection-specific training set.
% \autoref{tab:sota_cleandata}에서 \emph{E2E}와 \emph{SelfLoc} 항목은 \emph{Global Descriptors+Detected to Retrieval}에만 존재하는 항목이다.
% \emph{E2E}는 End-to-End 학습의 Single-Stage Pipeline 방법을 의미하고, Localization은 위치 정보가 필요한데 이를 필요치 않는 Unsupervised Learning방법을 \emph{SelfLoc}라 한다. 
% \emph{Global Descriptors+Detected to Retrieval} 연구들의 \emph{TrainSet} 항목을 보면, 다양한 학습셋을 적용했는데, 이는 Detection과 Retrieval이 동시에 annotation된 데이터셋이 없기 때문이다.
% 결과적으로, 우리는 Detection관련 학습셋이 필요없는 \emph{E2E}과 \emph{SelfLoc}조건에 맞는 유일한 연구라할 수 있다.

%------------------------------------------------------------------------------

\paragraph{New clean dataset, distractors}

\autoref{tab:1m} provides complete experimental results, including the impact of introducing 1 million distractors (\r 1m) into the evaluation set, on our new clean training set, $\cR$GLDv2-clean, as well as the previous most popular clean set, SfM-120k. Contrary to previous studies, we compare methods trained on the same training and evaluation sets to ensure fairness. \iavr{Well, yes, but we use $\mathbf{D2R}$ while other methods in this table do not. Whereas in the previous \autoref{tab:sota_cleandata}, we compare with other methods using $\mathbf{D2R}$, but not on the same dataset. We should really reproduce methods using $\mathbf{D2R}$ (\eg, DIR, R-ASMK) and compare with them on both SfM-120k and the new $\cR$GLDv2-clean. Also add them to \autoref{tab:sota2_diff}.}

% Some metrics under $\mathbf{S_{2}D2R}$ in {\rpa+\r1m} underperform, but 
Without fine-tuning, 
%our $\mathbf{S_{2}D2R}$, consistently outperforms previous SOTA on most metrics. We achieve an improvement of 5.1\% mAP on \rox$+$\r1m~(medium) and 2.5\% on \rox$+$\r1m~(hard).
\alert{we found improvements (mAP) of 1.3\% for \rox$+$\r1m~(medium), 5.1\% for \rox$+$\r1m~(hard), 1.7\% for \rpar$+$\r1m~(medium), and 0.8\% for \rpar$+$\r1m~(hard) compared to DOLG~\cite{yang2021dolg} on the $\cR$GLDv2-clean set.}
\iavr{Comparing to what in particular, and on which training set?} With fine-tuning, our $\mathbf{S_{2}D2R}$+$\Th{FT}$ establishes new SOTA results for nearly all tested metrics. In particular,
%we improve by 10.2\% on \rox$+$\r1m, 5.5\% on \rpar$+$\r1m (medium) and by 16.9\% on \rox$+$\r1m, 2.1\% on \rpar$+$\r1m (hard). 
\alert{we found improvements (mAP) of 4.5\% for \rox$+$\r1m~(medium), 5.3\% for \rox$+$\r1m~(hard), 4.3\% for \rpar$+$\r1m~(medium), and 3.1\% for \rpar$+$\r1m~(hard) compared to DOLG~\cite{yang2021dolg} on the $\cR$GLDv2-clean set.}
\iavr{Again, comparing to what, and on which training set?} 
\CH{I fixed both, including the previous one.}
%
% \autoref{sec:dataset} describes \emph{$\cR$GLDV2-clean}, a new dataset developed for this study. The results of applying the new data are shown in \Th{Global Descriptors+Revisiting GLDV2} in \autoref{tab:1m}. Although we attempted to reproduce previous SOTA algorithms, complete replication for all previous experiments, proved challenging. This is largely because \emph{$\cR$GLDV2-clean} requires a large amount of data (approximately 15 million), and many previous SOTA methods have not publicly disclosed their source codes. To ensure a fair evaluation, our experiments employed the same ResNet101 backbone~\cite{Gordo01, Kalantidis01, Radenovic01, gu2018attention, Ng01, Yokoo01, SCH01, yang2021dolg, tokens} and ArcFace loss~\cite{Yokoo01, SCH01, yang2021dolg, tokens, dtop} used in previous studies. Wherever possible, we used publicly available official codes. It is also worth noting that previous comparative evaluations often employed different training sets while using the same evaluation set, which could introduce bias. Our study, however, utilizes the same training and evaluation sets to ensure fairness. The results affirm that our method surpasses previous studies.
% 우리는 \autoref{sec:dataset}에서 우리의 새로운 데이터셋인 \emph{$\cR$GLDV2-clean}에 대한 설명을 하였다.
% \autoref{tab:sota_cleandata}의 \Th{Global Descriptors+Revisiting GLDV2}에서 새로운 데이터를 적용한 결과를 볼 수 있다.
% 우리는 이 실험을 위해서, 이전 SOTA 알고리즘을 리프로듀싱하였지만 이전의 모든 실험에 대해 완벽히 리프로듀싱하기는 어려움이 있다. 
% \autoref{tab:table2}에서 보듯이, \emph{$\cR$GLDV2-clean}는 약 15M장의 많은 데이터, 각각의 학습에 적용 된 다양한 Sampling 방식, 그리고 이전의 많은 SOTA 방법의 소스들 공개되지 않은 점 때문이다.
% %특히, 장비의 제약이 있었다. 학습에 이용한 장비는 \autoref{sec:Implementation}에서 확인할 수 있다. 
% % 특히, \autoref{sec:Implementation}에서 언급한 장비로는 제약이 있었다.
% 우리는 이러한 제약조건에서, 최대한 공정한 실험을 위해, 기존 연구들에서 가장 많이 적용된, Resnet101 backbone~\cite{Gordo01, Kalantidis01, Radenovic01, gu2018attention, Ng01, Yokoo01, SCH01, yang2021dolg, tokens}과 ArcFace loss~\cite{Yokoo01, SCH01, yang2021dolg, tokens, dtop}를 고정시켜 각 이전 연구에 적용되었던 네트워크들과 함께 \emph{$\cR$GLDV2-clean} 데이터셋를 적용시켜 실험한다. 
% 그리고 이전 연구에 적용되었던 네트워크들은 최대한 공개된 official code를 이용하였다.
% 또한, 이전 연구들의 비교 평가는 평가셋은 동일하지만, 다른 학습셋을 적용한 연구들과 비교한 경우들이다. 
% 이 점은 불공평한 평가 결과를 제공한다고 생각한다.
% 우리는 공평한 평가를 위해 학습셋과 평가셋을 동일하게 하여 실험하였다.
% %\autoref{tab:sota_cleandata}는 이에 대한 우리의 실험 결과를 보여준다.
% %이 실험 결과에서 우리가 제안한 방법이 이전 연구보다 더 뛰어난 성능을 보여주고 있다.
% 실험 결과에서 우리가 제안한 방법이 이전 연구보다 더 뛰어난 성능을 보여주고 있다.


==> tex/sec_exp_impl-1.tex <==
%------------------------------------------------------------------------------
\begin{table*}
\centering
\input{exp/exp_gldv2_clean_2_vs_filtered}
\vspace{-6pt}
\caption{Comparison of the original GLDv2-clean training set with our revisited version $\cR$GLDv2-clean for a number of SOTA methods that we reproduce with ResNet101 backbone, arcface loss and same sampling, settings and hyperparameters. $\dagger/\ddagger$: official/our code. \iavr{Did you actually reproduce the numbers of the original GLDv2-clean, or are they as published? If you did, we should have daggers everywhere. If not, that's trouble :-)} \CH{The absence of daggers is the result of experiments in each cited reference.}
}
\label{tab:sota2_diff}
\end{table*}
%------------------------------------------------------------------------------

\section{Experiments}
\label{sec:exp}

\subsection{Implementation}
\label{sec:impl}

\paragraph{Components}

Most instance-level image retrieval studies propose a kind of head on top of the backbone network that performs a particular operation to enhance retrieval performance. The same is happening independently in studies of category-level tasks like localization, even though the operations may be similar. Comparison is often challenging, when official code is not released. Our focus is on detection for retrieval in this work but we still need to compare with SOTA methods, which may perform different operations. We thus follow a neutral approach whereby we reuse existing, well-established components from the literature, introduced either for instance-level or category-level tasks.

In particular, given an input image $x \in \cX$, where $\cX$ is the image space, we obtain an embedding $\vu = f(x) \in \real^d$, where $d$ is the embedding dimension and
\begin{equation}
	f = f^p \circ f^\ell \circ f^c \circ f^e \circ f^b
\label{eq:map}
\end{equation}
is the composition of a number of functions. Here,
\begin{itemize}[itemsep=1pt, parsep=0pt, topsep=3pt]
	\item $f^b: \cX \to \real^{w \times h \times d}$ is the \emph{backbone network};
	\item $f^e: \real^{w \times h \times d} \to \real^{w \times h \times d}$ is \emph{backbone enhancement} (EB), including non-local interactions, such as ECNet~\cite{wang01}, NLNet~\cite{Wang02}, Gather-Excite~\cite{GatherExcite} or SENet~\cite{Hu01} \CH{Shouldn't it be BE instead of EB?}
	\item $f^c: \real^{w \times h \times d} \to \real^{w \times h \times d}$ is \emph{selective context} (SC), enriching contextual information to apply locality more effectively, such as ASPP~\cite{Chen2017RethinkingAC} or SKNet~\cite{sknet};
	\item $f^\ell: \real^{w \times h \times d} \to \real^{w \times h \times d}$ is our \emph{attentional localization} (AL) (\autoref{sec:1-stage}), localizing objects of interest in an unsupervised fashion;
	\item $f^p: \real^{w \times h \times d} \to \real^d$ is a \emph{spatial pooling} operation, such as GAP or GeM~\cite{Radenovic01}, optionally followed by other mappings, \eg whitening.
\end{itemize}
In the Appendix, we ablate different options for $f^e, f^c$ and we specify our choice for $f^p$; then in \autoref{sec:ablation} we ablate, apart from hyperparameters of $f^\ell$, the effect of the presence of components $f^e, f^c, f^\ell$ on the overall performance. By default, we embed images using $f$~\eq{map}, where for each component we use default settings as specified in \autoref{sec:ablation} or in the Appendix.

%------------------------------------------------------------------------------

\paragraph{Settings}

Certain existing works~\cite{Gordo01, delf} train the backbone network first on classification loss without the head corresponding to the method and then freeze the backbone and train the head only. We refer to this approach as ``fine-tuning'' (FT) and we give more details in the Appendix. 
% \autoref{fig:A5_FT}
To allow for comparisons, we train our model both with and without fine-tuning, in which case everything is trained in a single stage end-to-end. We refer to our method as \ours without fine-tuning and \oursf with fine-tuning. All experimental setings are detailed in the Appendix.
\CH{The difference between DIR and DELF is that the existing R101 backbone freezes when training. Figure A11/A12 illustrates this. Should we say 2 stage fine-tuning?}
\iavr{I thought it was clear but now I am not sure again. Your definition of FT is essentially fig A10, where in the second stage of FT (b), the backbone is frozen. Both DIR and DELF have ``Y'' in FT column of table. But here you are saying that in addition, the backbone is \textbf{not} frozen for both DIR and DELF? For which one is it frozen and for which not? Figures A11/A12 do nt say anything about this.}
\CH{DIR and DELF were not frozen. Only our study was frozen. That's the difference between the two studies, in this training method.}

==> tex/sec_exp_vis-1.tex <==
\subsection{Visualization}
\label{sec:Visualization}

%------------------------------------------------------------------------------
\begin{figure*}
\centering
\fig[.9]{5}
\vspace{-6pt}
\caption{Examples of top-5 ranking images retrieved by our $\mathbf{S_{2}D2R}$ model from evaluation sets \oxf5k/\paris6k and associated spatial attention map $A$~\eq{attn}. The red rectangle within the query on the left is the cropped area provided by the evaluation set and is actually used as the query image.
\CH{Since all the pictures are currently edited/saved in Google Slides, I'm a bit limited in this regard. And since I'm using a web tool to convert them to PDF, I have to convert them one by one. Since there are so many, this fig is limited because there are so many. Sorry, I can't do this or it will take some time.}
\iavr{No no no, you got me wrong. As I said, here we don't need pdf, just png/jpg, because it's just images. Then, you don't need Google slides. The ``Query'', ``Top-1'' etc. we do in Latex. We don't need red/blue boxes either. So, just save your original images, before putting them in Google slides.}
\CH{This image should come from Google Slides. I will notify you as soon as it is completed by tomorrow.}
\iavr{I do not understand. Don't you have the original images? How do you put them into Google slides? Can't you just put them into a folder instead?}
\CH{Sorry, I had a problem with the images in this Google Slides. 
I had these images in Google Slides, so I thought it was fine.
It's too late today, so I'll make sure to get this done by tomorrow.}
\CH{I uploaded all the images (f6\_*\_*\_*.png)
}
}
\label{fig:fig5}
\end{figure*}
%------------------------------------------------------------------------------

\paragraph{Ranking and spatial attention}

\autoref{fig:fig5} shows examples of the top-5 ranking images retrieved for a number of queries by our model, along with the associated spatial attention map. 
% The ranking results are derived from applying $\mathtt{\vF}$ in \autoref{eq:Bottleneck}. 
The spatial attention map $A$~\eq{attn} focuses exclusively on the object of interest as specified by the cropped area provided by the evaluation set, essentially ignoring the background.
% \autoref{fig:fig5}은 spatial attention map과 함께 우리 모델의 Top-5 Ranking 결과를 보여준다. 
% 이 그림에서, 왼쪽의 첫번째 그림은 Query를 의미하며, 그 이미지안의 Red Rectangle은 Oxford5k와 Paris6k이 제공하는 Cropped 영역으로 실제 쿼리 입력에 해당한다.
% Ranking 결과는 \autoref{eq:Bottleneck}의 $\mathtt{\vF}$를 적용한것이다.
% spatial attention map은 \autoref{eq:attn}의 $\vF^{s}$을 의미하며, 이는 명확히 background가 아닌 우리가 찾고자 하는 관심대상 (the object of interest)만 attend 하는 것을 볼 수 있다.

%------------------------------------------------------------------------------
\begin{figure}
\centering
% \fig{7}
\scriptsize
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ccc}
& Pre-trained & Ours \\
\raisebox{.16\columnwidth}{(a)} & \fig[.47]{7_1_1_crop} & \fig[.47]{7_1_2_crop} \\[-1pt]
\raisebox{.16\columnwidth}{(b)} & \fig[.47]{7_2_1_crop} & \fig[.47]{7_2_2_crop} \\[-1pt]
\raisebox{.16\columnwidth}{(c)} & \fig[.47]{7_3_1_crop} & \fig[.47]{7_3_2_crop} 
\end{tabular}
\vspace{-6pt}
\caption{T-SNE visualization of image embeddings of the \emph{revisited Paris} (\rpa) evaluation set under (a) \emph{easy}, (b) \emph{medium}, and (c) \emph{hard} protocols~\cite{RITAC18}. \alert{We compare our model learned on top of frozen ResNet101 as pre-trained on ImageNet with the same fine-tuned on the SfM-120k dataset~\cite{Radenovic01}.} \iavr{right?} \CH{right.} Positive images for each protocol are colored based on their query landmark category.
% The \emph{medium} (b) is formed by combining both \emph{easy} (a) and \emph{hard} (c).
\iavr{I cropped the png images myself. But, it should really be pdf in vector format.}
% Images cropped with
% 	for f in 7_*.png; do convert -trim $f `basename $f .png`_crop.png; done
}
\label{fig:fig5_embedding}
\end{figure}
%------------------------------------------------------------------------------

\paragraph{Embedding space}

\alert{\autoref{fig:fig5_embedding} shows t-SNE visualizations of image embeddings of the \rpar dataset~\cite{RITAC18}, obtained by our model learned on a frozen network \vs fine-tuning on SfM-120k~\cite{Radenovic01}.} \iavr{Is this right?} \CH{frozen network? This is just using the "pre-trained on ImageNet" feature.} \iavr{Sorry I though this is the same as in fig. 5, where you need our ``D2R'' part on top of the pre-trained backbone, which has to remain frozen, right? But here there is D2R part, so it's only the pre-trained backbone features, I guess with GeM, right? I will fix.} This visualization indicates superior embedding quality for our model. \iavr{If I get this right, we should really compare with a proper baseline that is fine-tuned but without ALM (and maybe without EBM or SCM). Comparing with off-the-shelf is not very interesting.}
\CH{Yep.  I put this in the Appendix.}


==> tex/sec_intro-1.tex <==
\vspace{-10pt}
\section{Introduction}
\label{sec:intro}

\begin{figure}[t]
\centering\includegraphics[width=1.0\columnwidth]{fig/f1.pdf}
%\end{center}
\vspace{-12pt}
\caption{ Two-Stage based Image Retrieval \vs Single-Stage based Image Retrieval (Ours)
\CH{Fixed the requested text. I changed the title of "stage2: embedding for Retrieval" to "embedding network" to mean a network that generates features for retrieval. I saved fig.1 as stage1(1\_p1.pdf), stage2(1\_p2.pdf).}
\iavr{Thanks. I think I asked you, what is ``embedding module'' in (b)? It sounds like something complex. Is it the ``refinement feature module'' (RFM) that is now in the appendix? Better not show this here. Better just say \eg ``Mask-based pooling'', referring to \eq{alm}. Also, remove the bounding box thing, just keep the mask. Because we don't use bounding boxes in ALM. Also, as I said before, ``1 :'' $\to$ ``1:'', ``2 :'' $\to$ ``2:''. Punctuation symbols take only one space after, not before.}
\CH{I fixed it to your request. 
And I wrote up the instructions in SLACK for creating the figure. 
Is this the resolution you want?}
}
\label{fig:fig1}
\end{figure}

Instance-level image retrieval (ILIR) is a significant area of research within deep learning, attracting substantial inquiry over the years. Previous research on ILIR generally falls into two categories: studies that focus on global descriptors and those that center on local descriptors. This study focuses on global descriptors, which offer notable computational advantages in search tasks compared to local descriptors such as SIFT~\cite{Lowe01}. Instead of scrutinizing what to identify within the feature map of a convolutional neural network (CNN), these studies examine how to effectively extract functional and efficient image features from feature map. Some studies ~\cite{Kalantidis01, Ng01, SCH01} have used attention information to incorporate spatial information as a way to improve feature extraction. However, a major limitation of existing methods is their inability to focus on a specific object when an image contains multiple objects. To overcome this, object detection ~\cite{fasterrcnn, yolo} techniques are often employed to isolate a specific object, which is then used as the input for image retrieval. These detected-to-retrieval ($\mathbf{D2R}$) approaches typically necessitate a complex two-stage pipeline training method as shown in (a) in \autoref{fig:fig1}, often requiring a separate training set. Contrarily, this study proposes a new more streamlined solution, utilizing a single-stage pipeline for learning, as illustrated in \autoref{fig:fig1} (b).
In addition to the modeling aspects suggested above, high-quality datasets are crucial for advancing research in deep learning, particularly in the field of ILIR. This area has benefited significantly from the availability of extensive landmark datasets \cite{Babenko01, Gordo01, Radenovic01, delf, Weyand01}. Among the published training sets, \emph{Neural Code Clean}~\cite{Gordo01} and SfM-120k~\cite{Radenovic01} stand out for their practice of excluding common categories between the training and evaluation sets to ensure a fair comparison. Meanwhile, GLDv2-clean ~\cite{Weyand01}, which has which has gained widespread recent use, has several problems.
% Instance Level Image Retrieval (ILIR)은 그 동안 Deep learning분야에서 하나의 중요한 task로써 많은 연구들이 진행되어 왔다.
% %특히, 여러 연구들에서부터 대용량의 랜드마크 데이터 셋 \cite{Babenko01, delf, Weyand01, Philbin01, Philbin02}들을 공개와 kaggle의 Google Landmark Retrieval\footnote {https://www.kaggle.com/c/landmark-retrieval-2021}에 의해 더욱더 활발히 연구가 진행되었다. 
% 이 ILIR 연구들은 크게 Global descriptor와 Local descriptor기반한 연구들로 나뉘어 구분할 수 있는데, 우리의 연구는 SIFT~\cite{Lowe01}같은 Local descriptor보다 검색 계산 비용에 훨씬 효율적인 Global descriptor에 관한 연구 주제로 진행된다.
% %현 시점에서, Global descriptnor와 관련된 이전 연구들은 Pooling 알고리즘 관점에서 수년간 집중적인 연구들이 진행되어 왔고, 현 상황에서 이들은 한계점에 이르렀다고 판단할 수 있다. 
% 이런 연구들은 CNN의 feature map안에서 찾고자하는 대상에 초점을 맞추기보다는, 그 feature map에서 기능적이고 효율적인 image feature를 추출하는 방법이다. %에 대한 연구라 할 수 있다.
% %또한, 
% 이러한 문제점을 해결하기 위한 방법으로 공간적 정보를 추가하기 위해 attention 정보를 이용하는 연구~\cite{Kalantidis01, Ng01, SCH01}들도 있었다.
% 하지만, 기존 방법들은 이미지 내에 여러 object가 있을 때 찾고자하는 특정 object에만 집중하지 못한다. 
% 그래서, 일반적으로 object detection~\cite{fasterrcnn, yolo}을 적용하여 특정 대상을 찾고, 그 찾은 대상을 입력값으로 하여 image retrieval를 수행한다.
% 이러한 Detected-to-Retrieval ($\mathbf{D2R}$)연구는 object detection를 수행하기 때문에, \autoref{fig:fig1}의 (a)처럼 2-stage Pipeline 학습 방법을 시도해야하고, 학습셋도 따로 준비해야하는 문제가 있다.
% 이에 반해, 우리는 \autoref{fig:fig1}의 (b) 그림과 같이 single-stage pipeline 학습 방법으로하는 새로운 해결책을 제시한다. 

% %그리고, ILIR은 여러 연구들에서부터 대용량의 랜드마크 데이터 셋 \cite{Babenko01, delf, Weyand01, Philbin01, Philbin02}들을 공개에 의해 활발히 연구가 진행된 요인중의 하나이다. 
% %우리는 이러한 공개된 데이터셋에 대한 문제를 제기하고 이에 대한 해결책을 제시한다.  
% 앞서 제안한 모델적인 측면 외, 양질의 데이터셋 역시 딥러닝 연구에 있어 필수적이다. ILIR 분야는 대용량 랜드마크 데이터셋 \cite{Babenko01, Gordo01, Radenovic01, delf, Weyand01} 공개에 의해 많은 진전을 이뤄왔다.
% 공개된 학습셋 중 \emph{Neural Code Clean}~\cite{Gordo01}과 SfM-120k~\cite{Radenovic01}은 공평한 비교를 위해, 학습셋과 평가셋사이에 공통된 카테고리가 제거하고 발표하였다. 반면에, 최근 가장 많이 사용하고 있는 GLDv2-Clean~\cite{Weyand01}은 몇가지 문제가 있음을 발견하였고, 이에 대한 해결책을 제시하려한다.
% %우리는 local descirptor와 End to End 아닌 연구들은 비교 연구에서 제외시킨다. 
% %즉, 이전 다른 연구들처럼 공평한 비교를 위해서 End to End 방식의 Global descritptor를 이용한 연구들과 비교한다. 

This study aims to address these issues and make the following contributions:
\begin{enumerate}[itemsep=2pt, parsep=0pt, topsep=0pt]
    \item
    We propose a method to remove common categories between the training and evaluation sets of GLDv2-clean, and present the resulting filtered dataset.
    \item 
    We present a $\mathbf{D2R}$ study that employs a single-stage method, allowing for end-to-end learning. This contrasts with traditional two-stage methods and is referred to as $\mathbf{S_{2}D2R}$ in our study. 
    \item 
    Our proposed $\mathbf{D2R}$ approach outperforms existing state-of-the-art (SOTA) models on existing datasets. Additionally, we demonstrate that our method also delivers superior SOTA performance on our newly released training set, outshining prior research.
  \end{enumerate}
% This study makes the following contributions:
% \begin{enumerate}[itemsep=2pt, parsep=0pt, topsep=0pt]
%     \item %공개된 학습셋중 \emph{Neural Code Clean}~\cite{Gordo01}과 SfM-120k~\cite{Radenovic01}은 공평한 비교를 위해, 학습셋과 평가셋사이에 공통된 카테고리가 제거하고 발표하였다. 반면에, 최근 가장 많이 사용하고 있는 GLDv2-Clean~\cite{Weyand01}은 그렇지 못하다는 것을 우리는 발견했다. 
%     본 연구는 GLDv2-Clean의 학습셋과 평가셋 사이의 공통된 카테고리를 제거하는 방법을 제시하고, 필터링된 데이터셋을 공개한다.         
%     \item %$\mathbf{D2R}$ 연구는 detecction과 retrieval 단계를 거치는 2-stage 방법이다. 
%     %이 방식은 데이터 구성 방법과 학습 비용이 많이 든다.
%     본 연구는 2-stage 방법이 아닌 End-to-End학습이 가능한 Single-Stage 방법의 $\mathbf{D2R}$ 연구를 제시한다 ($\mathbf{S_{2}D2R}$).
%     %따라서, 본 연구는 2-stage 방법이 아닌 Single-Stage 방법의 End-to-End기반의 $\mathbf{D2R}$ 연구를 제시한다 ($\mathbf{S_{2}D2R}$).
%     \item 우리가 제안한 $\mathbf{D2R}$ 연구는 기존 데이터셋에서 이전 다른 모델보다 뛰어난 SOTA 성능을 내었음을 보여준다.  
%     또한, 새롭게 공개된 학습셋에서도 우리가 제안한 방법이 이전 다른 연구보다 SOTA 성능을 내었음을 보여준다.
%   \end{enumerate}

==> tex/sec_intro-2.tex <==
\vspace{-10pt}
\section{Introduction}
\label{sec:intro}

\begin{figure}[t]
\centering
\fig{f1.pdf}
\vspace{-12pt}
\caption{It is beneficial for image retrieval to detect objects of interest in database images and only represent those. (a) \emph{Two-stage} pipeline. Previous works involve two-stage embedding extraction at indexing, or a two-stage training process, and they may use location supervision or not. (b) \emph{One-stage} pipeline. We use a single-stage embedding extraction at training and indexing; training is end-to-end and uses no location supervision.
\iavr{Thanks for the edits. Can you please also split the left and right parts in two files so that ``(a) ... (b)'' are done in latex? PDFs look like they are in vector format indeed.}
\CH{I split the figure.(f1\_left/f1\_right.pdf)}
}
\label{fig:fig1}
\end{figure}

Instance-level image retrieval (ILIR) is a significant area of research within deep learning, attracting substantial inquiry over the years. Previous research on ILIR generally falls into two categories: studies that focus on global descriptors and those that center on local descriptors. This study focuses on global descriptors, which offer notable computational advantages in search tasks compared to local descriptors such as SIFT~\cite{Lowe01}. Instead of scrutinizing what to identify within the feature map of a convolutional neural network (CNN), these studies examine how to effectively extract functional and efficient image features from feature map. Some studies ~\cite{Kalantidis01, Ng01, SCH01} have used attention information to incorporate spatial information as a way to improve feature extraction. However, a major limitation of existing methods is their inability to focus on a specific object when an image contains multiple objects. To overcome this, object detection ~\cite{fasterrcnn, yolo} techniques are often employed to isolate a specific object, which is then used as the input for image retrieval. These detected-to-retrieval ($\mathbf{D2R}$) approaches typically necessitate a complex two-stage pipeline training method as shown in (a) in \autoref{fig:fig1}, often requiring a separate training set. Contrarily, this study proposes a new more streamlined solution, utilizing a single-stage pipeline for learning, as illustrated in \autoref{fig:fig1} (b).
In addition to the modeling aspects suggested above, high-quality datasets are crucial for advancing research in deep learning, particularly in the field of ILIR. This area has benefited significantly from the availability of extensive landmark datasets \cite{Babenko01, Gordo01, Radenovic01, delf, Weyand01}. Among the published training sets, \emph{Neural Code Clean}~\cite{Gordo01} and SfM-120k~\cite{Radenovic01} stand out for their practice of excluding common categories between the training and evaluation sets to ensure a fair comparison. Meanwhile, GLDv2-clean ~\cite{Weyand01}, which has which has gained widespread recent use, has several problems.
% Instance Level Image Retrieval (ILIR)은 그 동안 Deep learning분야에서 하나의 중요한 task로써 많은 연구들이 진행되어 왔다.
% %특히, 여러 연구들에서부터 대용량의 랜드마크 데이터 셋 \cite{Babenko01, delf, Weyand01, Philbin01, Philbin02}들을 공개와 kaggle의 Google Landmark Retrieval\footnote {https://www.kaggle.com/c/landmark-retrieval-2021}에 의해 더욱더 활발히 연구가 진행되었다. 
% 이 ILIR 연구들은 크게 Global descriptor와 Local descriptor기반한 연구들로 나뉘어 구분할 수 있는데, 우리의 연구는 SIFT~\cite{Lowe01}같은 Local descriptor보다 검색 계산 비용에 훨씬 효율적인 Global descriptor에 관한 연구 주제로 진행된다.
% %현 시점에서, Global descriptnor와 관련된 이전 연구들은 Pooling 알고리즘 관점에서 수년간 집중적인 연구들이 진행되어 왔고, 현 상황에서 이들은 한계점에 이르렀다고 판단할 수 있다. 
% 이런 연구들은 CNN의 feature map안에서 찾고자하는 대상에 초점을 맞추기보다는, 그 feature map에서 기능적이고 효율적인 image feature를 추출하는 방법이다. %에 대한 연구라 할 수 있다.
% %또한, 
% 이러한 문제점을 해결하기 위한 방법으로 공간적 정보를 추가하기 위해 attention 정보를 이용하는 연구~\cite{Kalantidis01, Ng01, SCH01}들도 있었다.
% 하지만, 기존 방법들은 이미지 내에 여러 object가 있을 때 찾고자하는 특정 object에만 집중하지 못한다. 
% 그래서, 일반적으로 object detection~\cite{fasterrcnn, yolo}을 적용하여 특정 대상을 찾고, 그 찾은 대상을 입력값으로 하여 image retrieval를 수행한다.
% 이러한 Detected-to-Retrieval ($\mathbf{D2R}$)연구는 object detection를 수행하기 때문에, \autoref{fig:fig1}의 (a)처럼 2-stage Pipeline 학습 방법을 시도해야하고, 학습셋도 따로 준비해야하는 문제가 있다.
% 이에 반해, 우리는 \autoref{fig:fig1}의 (b) 그림과 같이 single-stage pipeline 학습 방법으로하는 새로운 해결책을 제시한다. 

% %그리고, ILIR은 여러 연구들에서부터 대용량의 랜드마크 데이터 셋 \cite{Babenko01, delf, Weyand01, Philbin01, Philbin02}들을 공개에 의해 활발히 연구가 진행된 요인중의 하나이다. 
% %우리는 이러한 공개된 데이터셋에 대한 문제를 제기하고 이에 대한 해결책을 제시한다.  
% 앞서 제안한 모델적인 측면 외, 양질의 데이터셋 역시 딥러닝 연구에 있어 필수적이다. ILIR 분야는 대용량 랜드마크 데이터셋 \cite{Babenko01, Gordo01, Radenovic01, delf, Weyand01} 공개에 의해 많은 진전을 이뤄왔다.
% 공개된 학습셋 중 \emph{Neural Code Clean}~\cite{Gordo01}과 SfM-120k~\cite{Radenovic01}은 공평한 비교를 위해, 학습셋과 평가셋사이에 공통된 카테고리가 제거하고 발표하였다. 반면에, 최근 가장 많이 사용하고 있는 GLDv2-Clean~\cite{Weyand01}은 몇가지 문제가 있음을 발견하였고, 이에 대한 해결책을 제시하려한다.
% %우리는 local descirptor와 End to End 아닌 연구들은 비교 연구에서 제외시킨다. 
% %즉, 이전 다른 연구들처럼 공평한 비교를 위해서 End to End 방식의 Global descritptor를 이용한 연구들과 비교한다. 

This study aims to address these issues and make the following contributions:
\begin{enumerate}[itemsep=2pt, parsep=0pt, topsep=0pt]
    \item
    We propose a method to remove common categories between the training and evaluation sets of GLDv2-clean, and present the resulting filtered dataset.
    \item 
    We present a $\mathbf{D2R}$ study that employs a single-stage method, allowing for end-to-end learning. This contrasts with traditional two-stage methods and is referred to as $\mathbf{S_{2}D2R}$ in our study. 
    \item 
    Our proposed $\mathbf{D2R}$ approach outperforms existing state-of-the-art (SOTA) models on existing datasets. Additionally, we demonstrate that our method also delivers superior SOTA performance on our newly released training set, outshining prior research.
  \end{enumerate}
% This study makes the following contributions:
% \begin{enumerate}[itemsep=2pt, parsep=0pt, topsep=0pt]
%     \item %공개된 학습셋중 \emph{Neural Code Clean}~\cite{Gordo01}과 SfM-120k~\cite{Radenovic01}은 공평한 비교를 위해, 학습셋과 평가셋사이에 공통된 카테고리가 제거하고 발표하였다. 반면에, 최근 가장 많이 사용하고 있는 GLDv2-Clean~\cite{Weyand01}은 그렇지 못하다는 것을 우리는 발견했다. 
%     본 연구는 GLDv2-Clean의 학습셋과 평가셋 사이의 공통된 카테고리를 제거하는 방법을 제시하고, 필터링된 데이터셋을 공개한다.         
%     \item %$\mathbf{D2R}$ 연구는 detecction과 retrieval 단계를 거치는 2-stage 방법이다. 
%     %이 방식은 데이터 구성 방법과 학습 비용이 많이 든다.
%     본 연구는 2-stage 방법이 아닌 End-to-End학습이 가능한 Single-Stage 방법의 $\mathbf{D2R}$ 연구를 제시한다 ($\mathbf{S_{2}D2R}$).
%     %따라서, 본 연구는 2-stage 방법이 아닌 Single-Stage 방법의 End-to-End기반의 $\mathbf{D2R}$ 연구를 제시한다 ($\mathbf{S_{2}D2R}$).
%     \item 우리가 제안한 $\mathbf{D2R}$ 연구는 기존 데이터셋에서 이전 다른 모델보다 뛰어난 SOTA 성능을 내었음을 보여준다.  
%     또한, 새롭게 공개된 학습셋에서도 우리가 제안한 방법이 이전 다른 연구보다 SOTA 성능을 내었음을 보여준다.
%   \end{enumerate}

==> tex/sec_method-1.tex <==
\begin{figure*}[t]
\begin{center}
	\fig[0.95]{3.png}
\end{center}
\vspace{-20pt}
\caption{ Single-Stage Detected-to-Retrieval ($\mathbf{S_{2}D2R}$) }
\label{fig:fig3}
\end{figure*}

%\vspace{-10pt}
\section{Single-Stage pipeline for $\mathbf{D2R}$ }
\label{sec:1-stage}

The motivation of this study is to deviate from the conventional two-stage D2R framework and introduce a unified, single-stage D2R method that integrates object detection. To achieve this, we propose a network architecture consisting of four modules that enable simultaneous instance detection and feature embedding for image retrieval, all within a singular network. The structure of this network is depicted in \autoref{fig:fig3}. 

\vspace{-10pt}
\paragraph{Two-Stage pipeline for $\mathbf{D2R}$}
From the perspective of ILIR, the key challenge in search performance is that target objects or instances are situated in different contexts within the image. One common solution is to use localization or object detection, which isolates the object from its background. These detected objects are then fed into the neural network to extract feature sets for image retrieval, as shown in \autoref{fig:fig1} (a). This approach comes with two main costs. First, in addition to the image retrieval dataset, a specialized training set that includes location and category information for the objects of interest is needed for the localization methods~\cite{fasterrcnn, yolo}. Second, the approach incurs higher costs because it operates as a two-stage method rather than an end-to-end process, as shown in \autoref{fig:fig1} (a).
This study presents a method to these problems. We replace the traditional localization step with a self-spatial attention mechanism, leveraging unsupervised learning. This allows us to solve for both $\mathbf{D2R}$ through a single, end-to-end learning process on a single backbone network, as illustrated in \autoref{fig:fig1} (b). Thus, the proposed method has the added advantage of eliminating the need for a specialized localization training set and the associated dual training cycles. Details of this approach are outlined in \autoref{sec:1-stage}.

\vspace{-10pt}
\paragraph{Attentional Localization Module (ALM)}

%\begin{figure}[t]
%\centering\includegraphics[width=0.85\columnwidth]%{fig/3_part2.png}
%\end{center}
%\vspace{-10pt}
%   \caption{ Attentional Localization Module %(ALM).
%   }
%\label{fig:ALM}
%\end{figure}
This module, depicted in \autoref{fig:fig1}(b) and elaborated in \autoref{fig:fig3}(b), is designed for instance detection. It employs a CNN-based self-spatial attention mechanism~\cite{Kalantidis01, delf, woo01}, which functions without the need for location supervision—hence, it is categorized as unsupervised learning. The feature map $\vF^{scm}$ generated by \autoref{eq:sknet}, serves as the input to the spatial attention module~\cite{delf}. The equation for this is as follows:

% \autoref{fig:fig1}의 (b)에서 Instance Detection 역할을 하는 모듈로, \autoref{fig:fig3}의 (b)에서 상세 그림을 보여주고 있다.
% 이를 위해 우리는 CNN기반의 Self Spatial Attention 메카니즘~\cite{Kalantidis01, delf, woo01}을 먼저 적용한다. 
% %우리는 어떠한 위치 정보를 주지 않고 학습하기 때문에 Unsupervised Learning이다. 
% 이는 위치에 대한 supervision 없이 학습하기 때문에 Unsupervised Learning이라 할 수 있다.
% 먼저 instance 위치 정보를 파악하기 위해, \autoref{eq:sknet}에서 생성된 feature map $\vF^{scm}$ 받아, Spatial Attention Module~\cite{delf}에 적용한다.
% 다음은 이에 대한 수식이다.

\begin{equation}
    \vF^{s} = \mathtt{MinMax}(\mathtt{softp}(\mathtt{Conv_{1 \times 1}}\left(\vF^{scm};\theta \right))) \in \real^{w \times h}
    \label{eq:delf}
\end{equation}

Here, $\mathtt{Conv_{1 \times 1}}$ is applied to $\vF^{scm}$ to reduce its dimensionality to 1. Subsequently, the softplus activation function ($\mathtt{softp}$) is applied. The generated $\vF^{s} \in \real^{w \times h \times 1}$ is a spatial attention map, which is used to acquire spatial information about the instance by learning. $\mathtt{MinMax}$ refers to min-max normalization. To identify the object region, we then apply:

% $\vF^{scm}$에 $\mathtt{Conv_{1 \times 1}}$를 적용하여 $D$ dimension을 1 dimension으로 전환한다. 
% %$\vF^{scm}$를 $\mathtt{Conv_{1 \times 1}}$를 이용하여 1 dimension으로 전환한다.
% 이후, softplus activation function ($\mathtt{softp}$)을 적용한다.  
% 여기서 생성된 $\vF^{s} \in \real^{w \times h \times 1}$는 spatial attention map이며, 이를 이용하여 instance에 대한 공간정보를 학습에 의해 획득하게 된다. 
% $\mathtt{MinMax}$는 min-max nomralized를 의미한다.
% 이후, Object 영역을 검출하기 위해 다음 수식을 적용한다. 

\begin{equation}\label{eq:binary}
%{AF}\left ( \mathit{s,c} \right ) = 
\vB_{m}  = 
\left\{
\begin{matrix}
B_{m}[x,y]  = \epsilon,  &  \mathit{if}\ \vF^{s}[x,y] < threshold_{i} \\ 
B_{m}[x,y]  = 1 , & else
\end{matrix}
\right.
\end{equation}
Here, $0 \leq m \leq M$, where $M$ denotes the number of predefined $0 \leq B_{m}[x,y] \leq 1$ values. $[x, y]$ denote the positions of the binary map. $\vB_{m}$ represents a binary map with the m-th threshold. In other words, $\vB_{m}$ contains the image information with the background removed. A value of 1 (foreground) is assigned if the pixel value surpasses a certain threshold, while 0 (background) is typically assigned otherwise. Unlike traditional static values, this study employs dynamic random values. Specifically, $0 \leq \epsilon \sim \mathcal{N}(0, 1) \leq 1$ denotes random noise sampled from a normal distribution, providing a probabilistic approach to background representation. \autoref{tab:bgvalue} shows the experimental results for this. \autoref{fig:fig4} shows the spatial information results of this. (a) shows the spatial attention map for the Resent101 model trained with just ImageNet. (b) refers to the spatial attention map $\vF^{s}$ in \autoref{eq:delf}, and (c) illustrates the binary map 
%(or localization map) 
$\vB$ given in \autoref{eq:binary}. (d) shows the region detected by applying the connected component labeling method using $\vB$, expressed as a blue square. Comparing (a) and (b) shows that the spatial attention map generated by the proposed model is much more attentive to the object being searched. These results show that the background is removed relatively well. 
%This binary map 
$\vB$ is obtained by unsupervised learning without any location information in the training set. $\vB$ is generated for the number of thresholds and fused with the feature map $\vF^{scm}$ generated using \autoref{eq:sknet}. At this time, each feature map is fused using the $\mathtt{H}$ function in \autoref{eq:fuse-bifpn}, mentioned above. The equation for this is as follows:
% 수식에서, $0 \leq m \leq M$ 이고, $M$은 미리 정의된 $0 \leq B_{m}[x,y] \leq 1$값을 가지는 threshold 개수를 의미한다.
% $x \in w$ 와 $y \in h$ 는 binary map의 위치를 의미한다. 
% $\vB_{m}$는 m번째 threshold를 이용한 Binary map 이다.
% 즉, $\vB_{m}$는 background를 제거된 이미지 정보를 담고 있다.
% 이 수식에서 threshold 이상일 경우는 1(foreground)을 주고, 그렇지 않는 경우에는 일반적으로 0 (background)을 준다.
% 하지만, 우리는 static값이 아닌 Random한 dynamic한 값을 주입한다.
% 수식에서 $0 \leq \epsilon \sim \mathcal{N}(0, 1) \leq 1$는 정규 분포에서 샘플링된 무작위 잡음을 나타내고, 이 분포에서 샘플링된 랜덤 노이즈를 background value로 준다.
% %실제 실험에서 0과 1 사이 구간에 존재하는 범위 값을 실험에 의해 결정한다. 
% \autoref{tab:bgvalue}은 이에 대한 실험 결과를 보여준다. 
% \autoref{fig:fig4}는 이에 대한 spatial information 결과를 보여준다. 
% (a)는 단지 ImageNet 으로 학습한 Resent101 모델에 대한 spatial attention map을 보여준다.
% (b)는 \autoref{eq:delf}의 Spatial attention map $\vF^{s}$를 의미하며, (c)는 \autoref{eq:binary}의 Binary Map (or Localization Map) $\vB$를 의미한다. 
% (d)는 $\vB$를 이용하여 connected component labeling 방법을 적용하여 감지한 detected region을 파란색 사각형으로 표현한 것이다. 
% % (a)는 단지 ImageNet 으로 학습한 Resent101 모델에 대한 spatial attention map을 보여준다.
% (a)와 (b)을 비교해볼때, 우리 모델에서 생성된 spatial attention map이  찾고자 하는 대상에 대해 훨씬 attend한다는 것을 보여준다.
% 이 결과에서, 비교적 잘 배경을 제거되는 결과를 볼 수 있다. 
% 그리고 이 Binary Map $\vB$는 학습셋에서 어떠한 위치 정보없이 Unsupervised Learning 방법으로 획득한 결과이다. 
% Threshold 개수에 맞게 $\vB$를 생성되고, 이들은 \autoref{eq:sknet}에서 생성된 feature map $\vF^{scm}$과 Fusing하게 된다.
% %이때, 앞서 설명한 \autoref{eq:fuse-bifpn}의 방법과 동일하게 learnable parameter를 이용하여 각 Feature map들을 Fusing을 하게 된다. 
% 이때, 앞서 설명한 \autoref{eq:fuse-bifpn}의 $\mathtt{H}$ 함수를 이용하여 각 Feature map들을 Fusing을 하게 된다.
% 다음은 이에 대한 수식이다. 

\begin{equation}
    \mathtt{\vF^{b}} = \mathtt{H}(\vB_{0}\odot\vF^{scm},\cdots,\vB_{M}\odot \vF^{scm};\theta) \in \real^{w \times h \times D}
\label{eq:fuse-bifpn2}
\end{equation}

where $\mathtt{\vF^{b}} $ is the fused feature map, and $\odot$ represents element-wise multiplication. \autoref{tab:thresholds} demonstrates the fusion efficacy with varying numbers of thresholds.
% 위 수식에서, $\mathtt{\vF^{b}} $ 은 Fusing 결과에서 나온 Feature map이다.
% $\odot$는 element wise multiplication이다.
% \autoref{tab:thresholds}은 threshold 개수에 따른 Fusing에 대한 실험 결과를 보여준다.

%
\input{exp/clean_datasets}
%
%\begin{table*}
%\centering
%\input{exp/exp_gldv2_clean3}
%\vspace{-8pt}
%\caption{
%mAP comparison of Previous studies \vs Ours using \emph{Filtered GLDV2-Clean}. $\dagger/\ddagger$: training using official/our code. Black bold: %best previous methods in block. Red: best results. Blue: Ours results higher than previous methods.
%}
%\label{tab:filtered_sota}
%\vspace{3pt}
%\end{table*}
%

\begin{figure}[t]
\centering\includegraphics[width=1.0\columnwidth]{fig/4.png}
%\end{center}
\vspace{-15pt}
   \caption{ Binary Map for background removing. left:spatial attention map. center:binary map. right:detected region (blue box). (a) is spatial attention map of pre-trained ResNet101 on ImageNet. (b),(c),(d) are our model. More examples of this can be found in Appendix \autoref{fig:fig5_add}.
   }
\label{fig:fig4}
\end{figure}



==> tex/sec_method-2.tex <==
\section{Single-stage pipeline for $\mathbf{D2R}$ }
\label{sec:1-stage}

%------------------------------------------------------------------------------
\begin{figure}
\centering
\fig[1.0]{f4}
\vspace{-6pt}
% \caption{Single-stage detect-to-retrieve ($\mathbf{S_{2}D2R}$).}
\caption{Attentional localization (AL). \iavr{Please make arrows smaller.} \CH{thin arrows and times font changed.}
\CH{I can't add Latex because I'm doing it in Google Slides.
I'm not sure what else to add. Since the old main fig is gone, do you want a more extended fig that can use two columns instead of one? I'm still thinking about it, but I can't come up with a good idea to expand it yet..... After- I fixed it a little bit, but the old original is still there in this image. If you don't like it, you can go back to the previous one.}
\iavr{Can you please go back to the previous layout? The fonts look too small here in one column, while in double column the figure is too large. Or at least, if you keep this layout, make fonts larger? You did add Latex symbols, how did you do that? They look ok, but can you also change $w_1, w_i, w_T$ to also use Latex? Can you also say $M_1, M_i, M_T$, consistently with the $w$'s? Finally, when I said make arrows smaller, I meant smaller arrow heads, not thinner lines. These arrow heads here look ok, but in the previous layout they were too large.}
\CH{Fixed some fonts and figures. and The arrow heads are out of my control.}
}
\label{fig:fig3}
\end{figure}
%------------------------------------------------------------------------------

% The motivation of this study is to deviate from the conventional two-stage D2R framework and introduce a unified, single-stage D2R method that integrates object detection. To achieve this, we propose a network architecture consisting of four modules that enable simultaneous instance detection and feature embedding for image retrieval, all within a singular network. The structure of this network is depicted in \autoref{fig:fig3}. 

%------------------------------------------------------------------------------

\paragraph{Motivation}

From the perspective of instance-level image retrieval, the key challenge is that target objects or instances are situated in different contexts within the image. One common solution is to use object localization or detection, isolating the objects of interest from the background. The detected objects are then used to extract an image representation for retrieval, as shown in \autoref{fig:fig1}(a). This \emph{two-stage} process can be applied to the indexed set, the queries, or both.

This approach comes with certain limitations. First, in addition to the training set for representation learning, a specialized training set is also required that is annotated with location information for the objects of interest~\cite{fasterrcnn, yolo}. Second, the two stages are often trained separately rather than end-to-end. Third, this approach incurs higher computational cost at indexing and search because it requires two forward passes through the network for each image.

In this work, we attempt to address these limitations. We replace the localization step with a \emph{spatial attention} mechanism, which does not require location supervision. This allows us to solve for both localization and representation learning through a single, end-to-end learning process on a single network, as illustrated in \autoref{fig:fig1}(b). This has the advantage of eliminating the need for a specialized training set for localization and the separate training cycles.

% %------------------------------------------------------------------------------
% \begin{figure}
% \centering
% \fig[.85]{3_part2.png}
% \end{center}
% \vspace{-10pt}
% \caption{ Attentional Localization Module %(ALM).}
% \label{fig:ALM}
% \end{figure}
% %------------------------------------------------------------------------------

\paragraph{Attentional localization (AL)}

This component, depicted in \autoref{fig:fig1}(b) and elaborated in \autoref{fig:fig3}, is designed for instance detection and subsequent image representation based on the detected objects. It employs a spatial attention mechanism~\cite{Kalantidis01, delf, woo01}, which does not need location supervision. Given a feature tensor $\vF \in \real^{w \times h \times d}$, where $w \times h$ is the spatial resolution and $d$ the feature dimension, we obtain the \emph{spatial attention map}
% The feature map $\vF^{scm}$ generated by \autoref{eq:sknet}, serves as the input to the spatial attention module~\cite{delf}.
%
% \autoref{fig:fig1}의 (b)에서 Instance Detection 역할을 하는 모듈로, \autoref{fig:fig3}의 (b)에서 상세 그림을 보여주고 있다.
% 이를 위해 우리는 CNN기반의 Self Spatial Attention 메카니즘~\cite{Kalantidis01, delf, woo01}을 먼저 적용한다. 
% %우리는 어떠한 위치 정보를 주지 않고 학습하기 때문에 Unsupervised Learning이다. 
% 이는 위치에 대한 supervision 없이 학습하기 때문에 Unsupervised Learning이라 할 수 있다.
% 먼저 instance 위치 정보를 파악하기 위해, \autoref{eq:sknet}에서 생성된 feature map $\vF^{scm}$ 받아, Spatial Attention Module~\cite{delf}에 적용한다.
% 다음은 이에 대한 수식이다.
%
\begin{equation}
	\vA = \eta(\zeta(f^\ell(\vF))) \in \real^{w \times h}.
\label{eq:attn}
\end{equation}

\CH{Here, it doesn't make sense to me that the addition of softmax is equivalent to the meaning of [CLS] in ViT. Why? Is it because the equation above is "self spatial attention"?
Also, the addition of softmax is something I tried once before in another study... but it didn't express the heat map well. (I may need more experiments) So, I added min-max. softmax belongs to regression, but I think it may be a kind of nomalization effect (0-1). So, isn't it similar?}
\iavr{$1 \times 1$ convolution is the same as the dot product of each patch feature with the weight vector of the convolution ``kernel'', which corresponds to the CLS embedding. Hence, it is the same as $QK\tran$ in transformers, where $Q$ is CLS and $K$ are the patches. Then, if we use softmax instead of ``softplus followed by $\ell_1$ normalization'', we get $A = \softmax(QK\tran)$. Next, if we don't do thresholding but multiply $A$ with $\vF$ directly, we get $\softmax(QK\tran) V$, where $V$ is $\vF$. Same as in transformers. This ``attention-based pooling'' is used for example in:
\begin{enumerate}
	\item Lee \etal ``Set Transformer: A Framework for Attention-based Permutation-Invariant Neural Networks'' (2019).
	\item Zhai \etal ``Scaling Vision Transformers'' (2021).
	\item Touvron \etal ``Augmenting Convolutional networks with attention-based aggregation'' (2021).
	\item Psomas \etal ``Keep It SimPool: Who Said Supervised Transformers Suffer from Attention Deficit?'' (2023) (my work).
	\item The ResNet encoder of CLIP.
\end{enumerate}
In 1-3, $Q$ is a learned parameter (as in our $1 \times 1$ convolution); in 4-5, $Q$ is obtained by GAP on the feature tensor. Comparing with such solutions is important. We should do that, at least as ablation.}

Here, $f^\ell$ is a simple mapping, for example a $1 \times 1$ convolutional layer that reduces dimension to 1, $\zeta(x) \defn \ln(1+e^x)$ for $x \in \real$ is the softplus function and
\begin{equation}
	\eta(X) \defn \frac{X - \min X}{\max X - \min X} \in \real^{w \times h}
\label{eq:minmax}
\end{equation}
linearly normalizes $X \in \real^{w \times h}$ to the interval $[0,1]$. To identify object regions, we then apply a sequence of thresholding operations, obtaining a corresponding sequence of masks
%
\begin{equation}
%{AF}\left ( \mathit{s,c} \right ) = 
M_i(\vp) = \left\{
	\begin{array}{ll}
		\beta,  & \mif\ A(\vp) < \tau_i \\ 
		1,      & \other
	\end{array}
\right.
\label{eq:mask}
\end{equation}
for $i \in \{1,\dots,T\}$. Here, $T$ is the number of masks, $\vp \in \{1,\dots,w\} \times \{1,\dots,h\}$ is the spatial position, $\tau_i \in [0,1]$ is the $i$-th threshold, $\beta$ is a scalar corresponding to background and $1$ corresponds to foreground.

Unlike a conventional fixed value like $\beta = 0$, we use a dynamic, randomized approach. In particular, for each $\vp$, we draw a sample $\epsilon \sim \cN(0,1)$ and we clip it to $[0,1]$ by defining $\beta = \min(0,\max(1,\epsilon))$. The motivation is that randomness compensates for incorrect predictions of the attention map~\eq{attn}, especially at an early stage of training. This choice is ablated in \autoref{tab:bgvalue}.

\autoref{fig:fig4} shows examples of attentional localization. Comparing (a) with (b) shows that the spatial attention map generated by our model is much more attentive to the object being searched than the pretrained network. These results show that the background is removed relatively well, despite not using any localization supervision at training.

The sequence of masks $B_1, \dots, B_T$~\eq{mask} is applied independently to the feature tensor $\vF$ and the resulting tensors are fused into a single tensor
%
% 수식에서, $0 \leq m \leq M$ 이고, $M$은 미리 정의된 $0 \leq B_{m}[x,y] \leq 1$값을 가지는 threshold 개수를 의미한다.
% $x \in w$ 와 $y \in h$ 는 binary map의 위치를 의미한다. 
% $\vB_{m}$는 m번째 threshold를 이용한 Binary map 이다.
% 즉, $\vB_{m}$는 background를 제거된 이미지 정보를 담고 있다.
% 이 수식에서 threshold 이상일 경우는 1(foreground)을 주고, 그렇지 않는 경우에는 일반적으로 0 (background)을 준다.
% 하지만, 우리는 static값이 아닌 Random한 dynamic한 값을 주입한다.
% 수식에서 $0 \leq \epsilon \sim \mathcal{N}(0, 1) \leq 1$는 정규 분포에서 샘플링된 무작위 잡음을 나타내고, 이 분포에서 샘플링된 랜덤 노이즈를 background value로 준다.
% %실제 실험에서 0과 1 사이 구간에 존재하는 범위 값을 실험에 의해 결정한다. 
% \autoref{tab:bgvalue}은 이에 대한 실험 결과를 보여준다. 
% \autoref{fig:fig4}는 이에 대한 spatial information 결과를 보여준다. 
% (a)는 단지 ImageNet 으로 학습한 Resent101 모델에 대한 spatial attention map을 보여준다.
% (b)는 \autoref{eq:attn}의 Spatial attention map $\vF^{s}$를 의미하며, (c)는 \autoref{eq:mask}의 Binary Map (or Localization Map) $\vB$를 의미한다. 
% (d)는 $\vB$를 이용하여 connected component labeling 방법을 적용하여 감지한 detected region을 파란색 사각형으로 표현한 것이다. 
% % (a)는 단지 ImageNet 으로 학습한 Resent101 모델에 대한 spatial attention map을 보여준다.
% (a)와 (b)을 비교해볼때, 우리 모델에서 생성된 spatial attention map이  찾고자 하는 대상에 대해 훨씬 attend한다는 것을 보여준다.
% 이 결과에서, 비교적 잘 배경을 제거되는 결과를 볼 수 있다. 
% 그리고 이 Binary Map $\vB$는 학습셋에서 어떠한 위치 정보없이 Unsupervised Learning 방법으로 획득한 결과이다. 
% Threshold 개수에 맞게 $\vB$를 생성되고, 이들은 \autoref{eq:sknet}에서 생성된 feature map $\vF^{scm}$과 Fusing하게 된다.
% %이때, 앞서 설명한 \autoref{eq:fuse-bifpn}의 방법과 동일하게 learnable parameter를 이용하여 각 Feature map들을 Fusing을 하게 된다. 
% 이때, 앞서 설명한 \autoref{eq:fuse-bifpn}의 $\mathtt{H}$ 함수를 이용하여 각 Feature map들을 Fusing을 하게 된다.
% 다음은 이에 대한 수식이다. 
%
\begin{equation}
	\vF^\ell = \mathtt{H}(M_1 \odot \vF, \dots, M_T \odot \vF) \in \real^{w \times h \times d},
\label{eq:alm}
\end{equation}
%
where $\odot$ denotes Hadamard product over spatial dimension, with broadcasting over the feature dimension. Fusion amounts to a learnable convex combination
\begin{equation}
    \mathtt{H}(\vF_1, \dots, \vF_T) = \frac{w_1 \vF_1 + \cdots + w_T \vF_T}{w_1 + \cdots + w_T},
\label{eq:fuse}
\end{equation}



where, for $i \in \{1,\dots,T\}$, the $i$-th weight is defined as $w_i = \zeta(\alpha_i)$ and $\alpha_i$ is a learnable parameter. \iavr{I replaced ReLU with softplus. This is more consistent with~\eq{attn} and does not need $\delta$ because all $w_i > 0$.} \iavr{But, DELF doesn't have any such fusion. Anyway, let's leave as it is now and we'll see later what to do. I suggest trying this in the experiment and keeping it if it works (at least with some low temperature). I would also try softmax. Please let me know if this is ok.} \CH{I hadn't thought of that. I just adopted the spatial attention part of the delf paper.} \CH{It's a little difficult in the current situation, but I'll try to do it at the next conference(?).} Thus, the importance of each threshold in localizing objects from the spatial attention map is implicitly learned from data, without supervision. \autoref{tab:thresholds} ablates the effect of the number $T$ of thresholds on the fusion efficacy.
% 위 수식에서, $\mathtt{\vF^{b}} $ 은 Fusing 결과에서 나온 Feature map이다.
% $\odot$는 element wise multiplication이다.
% \autoref{tab:thresholds}은 threshold 개수에 따른 Fusing에 대한 실험 결과를 보여준다.

% %------------------------------------------------------------------------------
% \begin{table*}
% \centering
% \input{exp/exp_gldv2_clean3}
% \vspace{-8pt}
% \caption{
% mAP comparison of Previous studies \vs Ours using \emph{Filtered GLDV2-Clean}. $\dagger/\ddagger$: training using official/our code. Black bold: %best previous methods in block. Red: best results. Blue: Ours results higher than previous methods.
% }
% \label{tab:filtered_sota}
% \vspace{3pt}
% \end{table*}
% %------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{figure}
\centering
% \fig[.99]{4}
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{cccc}
\fig[.24]{5_1_1} & \mc{3}{\fig[.72]{5_1_2}} \\[-1pt]
\fig[.24]{5_2_1} & \mc{3}{\fig[.72]{5_2_2}} \\[-1pt]
\fig[.24]{5_3_1} & \mc{3}{\fig[.72]{5_3_2}} \\[-1pt]
\fig[.24]{5_4_1} & \mc{3}{\fig[.72]{5_4_2}} \\[-1pt]
\fig[.24]{5_5_1} & \mc{3}{\fig[.72]{5_5_2}} \\
\makebox[.22\columnwidth][c]{(a) $A$, pre-trained} &
\makebox[.22\columnwidth][c]{(b) $A$, ours} & 
\makebox[.22\columnwidth][c]{(c) Mask $M_i$} & 
\makebox[.22\columnwidth][c]{(d) Bounding box} \\
\end{tabular}
\vspace{-6pt}
\caption{\emph{Attentional localization (AL)}. (a) Spatial attention map $A$~\eq{attn} learned on frozen ResNet101, as pre-trained on ImageNet. (b) Same, but with the network fine-tuned on $\cR$GLDv2-clean. (c) Binary mask $M_i$~\eq{mask}, with $\beta = 0$ for visualization. \iavr{Which $i$?} \CH{Yes.} \iavr{Sorry, I meant which $i$? Which threshold? There are $T$ of them.} (d) Detected regions as bounding boxes of connected components of $M_i$, overlaid on input image (in blue). More examples can be found in the Appendix.
% \autoref{fig:fig5_add}.
\iavr{It was painful to create the figure properly in Latex. For later, will you please modify your code to save each image separately? This should be much easier.}
}
\label{fig:fig4}
\end{figure}
%------------------------------------------------------------------------------



==> tex/sec_method-3.tex <==
\section{Single-stage pipeline for $\mathbf{D2R}$ }
\label{sec:1-stage}

%------------------------------------------------------------------------------
\begin{figure}
\centering
\fig[1.0]{f4}
\vspace{-12pt}
% \caption{Single-stage detect-to-retrieve ($\mathbf{S_{2}D2R}$).}
\caption{\emph{Attentional localization} (AL). Given a feature tensor $\vF \in \real^{w \times h \times d}$, we obtain a spatial attention map $A \in \real^{w \times h}$~\eq{attn} and we apply multiple thresholding operations to obtain a sequence of masks $M_1, \dots M_T$~\eq{mask}. The masks are applied independently to $\vF$ and the resulting tensors are fused into a single tensor $\vF^\ell$ by a convex combination with learnable weights $w_1, \dots, w_T$~\eq{alm}.} 
\label{fig:fig3}
\end{figure}
%------------------------------------------------------------------------------

% The motivation of this study is to deviate from the conventional two-stage D2R framework and introduce a unified, single-stage D2R method that integrates object detection. To achieve this, we propose a network architecture consisting of four modules that enable simultaneous instance detection and feature embedding for image retrieval, all within a singular network. The structure of this network is depicted in \autoref{fig:fig3}. 

%------------------------------------------------------------------------------

\paragraph{Motivation}

From the perspective of instance-level image retrieval, the key challenge is that target objects or instances are situated in different contexts within the image. One common solution is to use object localization or detection, isolating the objects of interest from the background. The detected objects are then used to extract an image representation for retrieval, as shown in \autoref{fig:fig1}(a). This \emph{two-stage} process can be applied to the indexed set, the queries, or both.

This approach comes with certain limitations. First, in addition to the training set for representation learning, a specialized training set is also required that is annotated with location information for the objects of interest~\cite{fasterrcnn, yolo}. Second, the two stages are often trained separately rather than end-to-end. Third, this approach incurs higher computational cost at indexing and search because it requires two forward passes through the network for each image.

In this work, we attempt to address these limitations. We replace the localization step with a \emph{spatial attention} mechanism, which does not require location supervision. This allows us to solve for both localization and representation learning through a single, end-to-end learning process on a single network, as illustrated in \autoref{fig:fig1}(b). This has the advantage of eliminating the need for a specialized training set for localization and the separate training cycles.

% %------------------------------------------------------------------------------
% \begin{figure}
% \centering
% \fig[.85]{3_part2.png}
% \end{center}
% \vspace{-10pt}
% \caption{ Attentional Localization Module %(ALM).}
% \label{fig:ALM}
% \end{figure}
% %------------------------------------------------------------------------------

\paragraph{Attentional localization (AL)}

This component, depicted in \autoref{fig:fig1}(b) and elaborated in \autoref{fig:fig3}, is designed for instance detection and subsequent image representation based on the detected objects. It employs a spatial attention mechanism~\cite{Kalantidis01, delf, woo01}, which does not need location supervision. Given a feature tensor $\vF \in \real^{w \times h \times d}$, where $w \times h$ is the spatial resolution and $d$ the feature dimension, we obtain the \emph{spatial attention map}
% The feature map $\vF^{scm}$ generated by \autoref{eq:sknet}, serves as the input to the spatial attention module~\cite{delf}.
%
% \autoref{fig:fig1}의 (b)에서 Instance Detection 역할을 하는 모듈로, \autoref{fig:fig3}의 (b)에서 상세 그림을 보여주고 있다.
% 이를 위해 우리는 CNN기반의 Self Spatial Attention 메카니즘~\cite{Kalantidis01, delf, woo01}을 먼저 적용한다. 
% %우리는 어떠한 위치 정보를 주지 않고 학습하기 때문에 Unsupervised Learning이다. 
% 이는 위치에 대한 supervision 없이 학습하기 때문에 Unsupervised Learning이라 할 수 있다.
% 먼저 instance 위치 정보를 파악하기 위해, \autoref{eq:sknet}에서 생성된 feature map $\vF^{scm}$ 받아, Spatial Attention Module~\cite{delf}에 적용한다.
% 다음은 이에 대한 수식이다.
%
\begin{equation}
	A = \eta(\zeta(f^\ell(\vF))) \in \real^{w \times h}.
\label{eq:attn}
\end{equation}
Here, $f^\ell$ is a simple mapping, for example a $1 \times 1$ convolutional layer that reduces dimension to 1, $\zeta(x) \defn \ln(1+e^x)$ for $x \in \real$ is the softplus function and
\begin{equation}
	\eta(X) \defn \frac{X - \min X}{\max X - \min X} \in \real^{w \times h}
\label{eq:minmax}
\end{equation}
linearly normalizes $X \in \real^{w \times h}$ to the interval $[0,1]$. To identify object regions, we then apply a sequence of thresholding operations, obtaining a corresponding sequence of masks
\begin{equation}
M_i(\vp) = \left\{
	\begin{array}{ll}
		\beta,  & \mif\ A(\vp) < \tau_i \\ 
		1,      & \other
	\end{array}
\right.
\label{eq:mask}
\end{equation}
for $i \in \{1,\dots,T\}$. Here, $T$ is the number of masks, $\vp \in \{1,\dots,w\} \times \{1,\dots,h\}$ is the spatial position, $\tau_i \in [0,1]$ is the $i$-th threshold, $\beta$ is a scalar corresponding to background and $1$ corresponds to foreground.

Unlike a conventional fixed value like $\beta = 0$, we use a dynamic, randomized approach. In particular, for each $\vp$, we draw a sample $\epsilon$ from a normal distribution and we clip it to $[0,1]$ by defining $\beta = \min(0,\max(1,\epsilon))$. The motivation is that randomness compensates for incorrect predictions of the attention map~\eq{attn}, especially at an early stage of training. This choice is ablated in \autoref{tab:bgvalue}.

\autoref{fig:fig4} shows examples of attentional localization. Comparing (a) with (b) shows that the spatial attention map generated by our model is much more attentive to the object being searched than the pretrained network. These results show that the background is removed relatively well, despite not using any localization supervision at training.

The sequence of masks $M_1, \dots, M_T$~\eq{mask} is applied independently to the feature tensor $\vF$ and the resulting tensors are fused into a single tensor
%
% 수식에서, $0 \leq m \leq M$ 이고, $M$은 미리 정의된 $0 \leq B_{m}[x,y] \leq 1$값을 가지는 threshold 개수를 의미한다.
% $x \in w$ 와 $y \in h$ 는 binary map의 위치를 의미한다. 
% $\vB_{m}$는 m번째 threshold를 이용한 Binary map 이다.
% 즉, $\vB_{m}$는 background를 제거된 이미지 정보를 담고 있다.
% 이 수식에서 threshold 이상일 경우는 1(foreground)을 주고, 그렇지 않는 경우에는 일반적으로 0 (background)을 준다.
% 하지만, 우리는 static값이 아닌 Random한 dynamic한 값을 주입한다.
% 수식에서 $0 \leq \epsilon \sim \mathcal{N}(0, 1) \leq 1$는 정규 분포에서 샘플링된 무작위 잡음을 나타내고, 이 분포에서 샘플링된 랜덤 노이즈를 background value로 준다.
% %실제 실험에서 0과 1 사이 구간에 존재하는 범위 값을 실험에 의해 결정한다. 
% \autoref{tab:bgvalue}은 이에 대한 실험 결과를 보여준다. 
% \autoref{fig:fig4}는 이에 대한 spatial information 결과를 보여준다. 
% (a)는 단지 ImageNet 으로 학습한 Resent101 모델에 대한 spatial attention map을 보여준다.
% (b)는 \autoref{eq:attn}의 Spatial attention map $\vF^{s}$를 의미하며, (c)는 \autoref{eq:mask}의 Binary Map (or Localization Map) $\vB$를 의미한다. 
% (d)는 $\vB$를 이용하여 connected component labeling 방법을 적용하여 감지한 detected region을 파란색 사각형으로 표현한 것이다. 
% % (a)는 단지 ImageNet 으로 학습한 Resent101 모델에 대한 spatial attention map을 보여준다.
% (a)와 (b)을 비교해볼때, 우리 모델에서 생성된 spatial attention map이  찾고자 하는 대상에 대해 훨씬 attend한다는 것을 보여준다.
% 이 결과에서, 비교적 잘 배경을 제거되는 결과를 볼 수 있다. 
% 그리고 이 Binary Map $\vB$는 학습셋에서 어떠한 위치 정보없이 Unsupervised Learning 방법으로 획득한 결과이다. 
% Threshold 개수에 맞게 $\vB$를 생성되고, 이들은 \autoref{eq:sknet}에서 생성된 feature map $\vF^{scm}$과 Fusing하게 된다.
% %이때, 앞서 설명한 \autoref{eq:fuse-bifpn}의 방법과 동일하게 learnable parameter를 이용하여 각 Feature map들을 Fusing을 하게 된다. 
% 이때, 앞서 설명한 \autoref{eq:fuse-bifpn}의 $\mathtt{H}$ 함수를 이용하여 각 Feature map들을 Fusing을 하게 된다.
% 다음은 이에 대한 수식이다. 
%
\begin{equation}
	\vF^\ell = \mathtt{H}(M_1 \odot \vF, \dots, M_T \odot \vF) \in \real^{w \times h \times d},
\label{eq:alm}
\end{equation}
%
where $\odot$ denotes Hadamard product over spatial dimension, with broadcasting over the feature dimension. Fusion amounts to a learnable convex combination
\begin{equation}
    \mathtt{H}(\vF_1, \dots, \vF_T) = \frac{w_1 \vF_1 + \cdots + w_T \vF_T}{w_1 + \cdots + w_T},
\label{eq:fuse}
\end{equation}
where, for $i \in \{1,\dots,T\}$, the $i$-th weight is defined as $w_i = \zeta(\alpha_i)$ and $\alpha_i$ is a learnable parameter. Thus, the importance of each threshold in localizing objects from the spatial attention map is implicitly learned from data, without supervision. \autoref{tab:thresholds} ablates the effect of the number $T$ of thresholds on the fusion efficacy.
% 위 수식에서, $\mathtt{\vF^{b}} $ 은 Fusing 결과에서 나온 Feature map이다.
% $\odot$는 element wise multiplication이다.
% \autoref{tab:thresholds}은 threshold 개수에 따른 Fusing에 대한 실험 결과를 보여준다.

% %------------------------------------------------------------------------------
% \begin{table*}
% \centering
% \input{exp/exp_gldv2_clean3}
% \vspace{-8pt}
% \caption{
% mAP comparison of Previous studies \vs Ours using \emph{Filtered GLDV2-Clean}. $\dagger/\ddagger$: training using official/our code. Black bold: %best previous methods in block. Red: best results. Blue: Ours results higher than previous methods.
% }
% \label{tab:filtered_sota}
% \vspace{3pt}
% \end{table*}
% %------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{figure}
\centering
% \fig[.99]{4}
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{cccc}
\fig[.24]{5_1_1} & \mc{3}{\fig[.72]{5_1_2}} \\[-1pt]
\fig[.24]{5_2_1} & \mc{3}{\fig[.72]{5_2_2}} \\[-1pt]
\fig[.24]{5_3_1} & \mc{3}{\fig[.72]{5_3_2}} \\[-1pt]
\fig[.24]{5_4_1} & \mc{3}{\fig[.72]{5_4_2}} \\[-1pt]
\fig[.24]{5_5_1} & \mc{3}{\fig[.72]{5_5_2}} \\
\makebox[.22\columnwidth][c]{(a) $A$, pre-trained} &
\makebox[.22\columnwidth][c]{(b) $A$, ours} & 
\makebox[.22\columnwidth][c]{(c) Mask $M_i$} & 
\makebox[.22\columnwidth][c]{(d) Bounding box} \\
\end{tabular}
\vspace{-6pt}
\caption{\emph{Attentional localization (AL)}. (a) Spatial attention map $A$~\eq{attn} learned on frozen ResNet101, as pre-trained on ImageNet. (b) Same, but with the network fine-tuned on $\cR$GLDv2-clean. (c) Binary mask $M_i$~\eq{mask}, with $\beta = 0$ for visualization. \iavr{Which $i$?} \CH{Yes.} \iavr{Sorry, I meant which $i$? Which threshold? There are $T$ of them.} (d) Detected regions as bounding boxes of connected components of $M_i$, overlaid on input image (in blue). More examples can be found in the Appendix.
% \autoref{fig:fig5_add}.
\iavr{It was painful to create the figure properly in Latex. For later, will you please modify your code to save each image separately? This should be much easier.}
\CH{I'm definitely going to do it that way for my next study. By all means !!!  }
}
\label{fig:fig4}
\end{figure}
%------------------------------------------------------------------------------



==> tex/sec_motivations.tex <==
 \begin{figure*}[t]
\begin{center}
	\fig[1.0]{2.png}
\end{center}
\vspace{-18pt}
\caption{Confirming overlapping categories between evaluation sets (Oxford5k, Paris6k) and training sets (GLDV2-Clean, NC-Clean, SfM-120k).  Green Box: Top-5 results for Oxford5k Query. Blue Box: Top-5 results for Paris6k. The first image inside each box is the query image (evaluation sets), represented by a red rectangle. Each box shows the top-5 results in the order of GLDV2-Clean, NC-Clean, SfM-120k. The pink box means landmarks that are identical to the query. 
More examples of this can be found in Appendix \autoref{fig:fig2_sup}.
}
\label{fig:fig2}
\end{figure*}
\vspace{-5pt}
\section{Two Motivations}
\label{sec:relatedworks}

%\subsection{Unfair training set : Revisiting Goolge landmark Dataset V2}
\vspace{-3pt}
\subsection{Unfaired Landmark Clean Trainset}
\label{sec:Unfair_dataset}

현재 ILIR 분야에서의 Landmark 데이터셋의 큰 특징은 학습셋과 평가셋이 여러 연구들에 의해서 각각 독립적으로 수집되어 공개되었다는 점이다. 
%즉, 학습셋과 평가셋은 동일한 연구자가 오픈한 것이 아니라, 각각 다른 연구자들이 수집하여 공개해왔다.
평가셋은 Oxford5k (\oxf5k)~\cite{Philbin01} 과 Paris6k (\paris6k)~\cite{Philbin02}데이터 셋을 이용하며, 최근에는 Revisited Oxford (\roxf~or \rox) 와 Paris (\rpar~or \rpa)~\cite{RITAC18}를 사용한다.
반면에, 학습셋은 각 연구들이 공개된 시기에 맞추어 각각 공개되었다. 
즉, \emph{Neural Code} (NC)~\cite{Babenko01}, \emph{Neural Code clean} (NC-clean)~\cite{Gordo01}, SfM-120k~\cite{Radenovic01}, Google Landmarks V1 (GLDv1)~\cite{delf}, Google Landmarks V2 (GLDv2 and GLDv2-clean)~\cite{Weyand01} 순서로 공개되어 현재 많은 관련 연구들에서 적용되고 있다. 
이들은 이미지 수가 초기에 수만단위로 출발해서 현재 수백만 단위의 데이터셋으로 확장하여 공개되었다. 
%
특히, 이 중 먼저 공개된 두 학습셋인 NC-clean과 SfM-120k 학습셋은 \emph{Clean} 셋으로써 크게 2개의 기준으로 공개되었다. 
%
첫번째, 데이터셋은 구글같은 검색 엔진에서 텍스트 키워드를 통해 수집했기 때문에, 이는 특정 원하는 landmark를 포함한 이외의 다양한 Noisy 이미지들을 당연히 포함하게 된다. 
대표적인 데이터셋은 NC, GLDv1, GLDv2 이다. 
이들은 \emph{Noisy} dataset이라고 불린다. 
반대로, Clean Dataset이라고 불리는 NC-clean, SfM-120k, GLDv2-Clean 들이 있다.
이들 Clean Dataset은 정규 학습셋으로 많이 사용되고 있고, 같은 클래스안에 같은 landmark (Instance)만 포함되어 있도록 다양한 방법~\cite{Gordo01, Radenovi01}을 통해서 필터링하였다. 
%
두번째, NC-clean과 SfM-120k 학습셋과 평가셋 (Oxford5k, Paris6k)은 중복 랜드마크가 없도록 필터링하여 공개했다는 점이다. 
즉, 이는 평가셋과 학습셋은 서로 overlapping된 landmark 클래스가 존재하지 않아야 한다는 점이다. 
하지만, 최근 가장 많이 사용하고 있는 GLDv2-clean 학습셋은 첫번째 조건은 부합하지만, 두번째 조건에는 부합하지 않다는데 그 문제점이 있다.  
이는 본 연구뿐만 아니라 다른 다양한 이전 연구~\cite{superfeatures}와 공개 커뮤니티\footnote{https://github.com/MCC-WH/Token/issues/1}에서 이러한 문제를 제기하고 있다. 
이는 다른 NC-clean과 SfM-120k 학습셋를 적용한 연구들의 결과와의 비교에서 공평하지 않다는 것을 의미한다.
즉, GLDv2-clean 학습셋으로 학습된 연구들은 NC-clean과 SfM-120k로 학습한 연구들보다도 평가에 있어서 \emph{inflated accuracy}를 보여준다는 것이다. 
본 연구는 이점에 대한 해결책을 제시하여 \autoref{sec:RevisitingGLDV2}에서 그 방법에 대해 기술한다.
마지막으로, 우리는 이 수정된 새로운 데이터셋을 공개한다. 

\subsection{Two-Stage pipeline for Detected to Retrieval}
\label{sec:2-Stage}

%ILIR 관점에서 검색 성능에서의 가장 문제점은 찾고자 하는 대상(Object or Instance)이 이미지 안에 다양한 Context(view, size, resolution, illumination, background, etc.)로 존재한다는 것이다.
ILIR 관점에서 검색 성능에서의 가장 문제점은 찾고자 하는 대상(Object or Instance)이 이미지 안에 다양한 Context에 놓여있다는 점이다.
%즉, 이미지안의 그 대상은 다양한 컨디션(view, size, resolution, illumination, background, etc.)이 존재한다.
%이 중 가장 큰 문제점중의 하나는 다양한 Context을 가진 background가 존재한다는 점이고, 이는 검색 성능을 저하시킨다. 
이러한 문제를 해결하기 위해, Localization (or Object Detection) 과정을 통해 background 영역이 제거된  이미지안의 Object만을 감지할 수 있다. 
이후,이를 이미지 embedding feature를 추출하기 위한 네트워크의 입력값으로 적용하게 된다.
\autoref{fig:fig1}의 (a)는 이에 대한 과정을 설명하고 있다.
이는 크게 두가지 큰 비용을 감수해야하는 것을 의미한다.
첫번째, 이미지 검색을 위한 데이터셋 이외에, Localization방법~\cite{fasterrcnn, yolo}을 채용하기 위해서, 찾고자하는 대상에 대한 위치정보와 카테고리 정보를 포함하는 학습셋이 추가로 필요하다는 의미이다. 
%이러한 데이터셋을 구성하기 위해서 많은 비용이 드는것은 당연한다.
%이는 그 데이터셋 구성에대한 대한 비용이 수반되는 것을 의미한다.
두번째, \autoref{fig:fig1}의 (a)에서 보듯, End-to-End가 아닌 2-stage 방법이기 때문에, 이에 대한 비용들이 당연히 추가된다. 

우리는 이러한 문제점을 해결하기 위한 방법을 제시한다. 
%\autoref{fig:fig1}의 (b) 처럼, Localization 파트를 대체하는 방법으로 우리는 Unsupervised Learning방법으로 CNN의 Self Spatial attention 메카니즘과 Image retrieval 을 위한 embedding network를 단일 백본에서 처리하는 End-to-End 방식을 제안한다.
\autoref{fig:fig1}의 (b) 처럼, Unsupervised Learning기반의 self spatial attention 메카니즘을 통해 Localization을 대체하는 방법과 Image retrieval 을 위한 embedding network를 오직 단일 백본에서  동시에 모두 처리하는 End-to-End 방식을 제안한다.
이 제안된 방식은 앞서 문제 제기된 Localization 학습셋 구성과 두 번의 학습과정 불필요하다는 것을 의미한다.
\autoref{sec:1-stage}에서 이에 대한 방법을 기술한다.


==> tex/sec_motivations_jy.tex <==
 \begin{figure*}[t]
\begin{center}
	\fig[0.95]{2.png}
\end{center}
\vspace{-19pt}
\caption{Confirming overlapping categories between evaluation sets (Oxford5k, Paris6k) and training sets (GLDV2-Clean, NC-Clean, SfM-120k).  Green Box: Top-5 results for Oxford5k Query. Blue Box: Top-5 results for Paris6k. The first image inside each box is the query image (evaluation sets), represented by a red rectangle. Each box shows the top-5 results in the order of GLDV2-Clean, NC-Clean, SfM-120k. The pink box means landmarks that are identical to the query. 
More examples of this can be found in Appendix \autoref{fig:fig2_sup}.
}
\label{fig:fig2}
\end{figure*}


==> tex/sec_related-1.tex <==
\section{Related Works}
\label{sec:relatedworks}

\paragraph{Instance Level Image Retrieval (ILIR)}

The field of image retrieval is generally divided into two parts: local descriptors (LD)~\cite{delf, Teichmann01, Oriane, Weyand01, Donoser01, Iscen_2017_CVPR, Yang01, Teichmann01} and global descriptors (GD)~\cite{Babenko01, Gordo01, Kalantidis01, Weyand01, Babenko03, Radenovic01, SCH01,yang2021dolg, dtop}. Research on LD has been applied to image retrieval before deep learning era, where methods like SIFT~\cite{Lowe01} were frequently employed. Given that multiple features are generated for each image in LD-based approaches, various aggregation methods~\cite{Philbin01, JPD+11, TAJ13} have been applied. Deep learning extensions of these concepts include studies such as DELF~\cite{delf}, DELG~\cite{cao2020unifying}, and those applying ASMK~\cite{Teichmann01, tolias2020learning}. 
\alert{In particular, DELF is similar to our work in that it uses spatial attention without location supervision, but differs in that it uses it in LD.}
In contrast, GD is more useful as it only generates a single, unified feature from an image, simplifying the retrieval process. 
%GD-focused research has leveraged a variety of pooling techniques—such as MAC~\cite{Razavian2015VisualIR}, SPoC~\cite{Babenko03}, CroW~\cite{Kalantidis01}, RMAC~\cite{ToliasSJ15, Gordo01}, and GeM~\cite{Radenovic01}—to extract meaningful information from the three-dimensional feature map extracted from the CNN backbones.
GD focused research has leveraged a variety of pooling techniques~\cite{Razavian2015VisualIR, Radenovic01, Babenko03, Kalantidis01, ToliasSJ15, Gordo01, Radenovic01} to extract meaningful information from the three-dimensional feature map extracted from the CNN backbones. 
Alternatively, some studies have attempted to combine LDs and GDs, achieving performance that surpasses GD alone approaches. However, these hybrid methods come with a drawback: they are computationally expensive. 
%They typically identify the top-k matches using GD and then re-rank these using LD, leading to higher search costs.
They identify the top-k matches using GD and then re-rank these using LD, leading to higher search costs.
\iavr{Can you add that our method is similar to DELF in that it obtains an attention map without supervision, but targets regions rather than local features?}
\CH{I added this just above, is this what you mean?}
% %이 분야는 크게 두 파트로 분류할 수 있는데, 이를 Global Descriptor (GD)~\cite{Babenko01, Gordo01, Kalantidis01, Weyand01, Babenko03, Radenovic01, SCH01,yang2021dolg, dtop} 와 Local Descriptor (LD)~\cite{delf, Teichmann01, Oriane, Weyand01, Donoser01, Iscen_2017_CVPR, Yang01, Teichmann01}로 나뉠 수 있다.
% %LD 에 비해, GD는 이미지 한장으로부터 단일 Image Feature만을 생성하기 때문에, 상대적으로 효용성이 크다. 
% %특히, GD관련 연구는  CNN backbone으로 부터 추출한 3차원의 feature map에 대해  MAC~\cite{Razavian2015VisualIR}, SPoC~\cite{Babenko03}, CroW~\cite{Kalantidis01}, RMAC~\cite{ToliasSJ15, Gordo01}, GeM~\cite{Radenovic01}같은 다양한 Pooling 기법를 적용하며 진행되어 왔다. 
% %LD의 연구는 Deep learning 이전에 대표적으로 SIFT~\cite{Lowe01}를 이용하여 image retrieval에 적용해왔다. 
% %이들은 한 이미지당 다수의 feature가 발생되기 때문에, 이들을 aggregation 하는 방법~\cite{Philbin01, JPD+11, TAJ13}을 적용하였다. 
% %이 개념을 Deep learning에 확장한 연구인 DELF~\cite{delf}, DELG~\cite{cao2020unifying}, ASMK을 응용한 연구들~\cite{Teichmann01, tolias2020learning}이 있다. 
% %또 다른 방법으로, LD는 GD과 조합하여 사용할 수 있다.
% %이는 검색 비용이 많이 들기 때문에, GD를 통해 Top-K를 찾고, 그 안에서 LD로 re-ranking을 한다. 
% %%Top-K만 하는 이유는 Query와 모든 DB사의 거리 측정은 매우 큰 비용이 들기 때문이다.
% %이 같은 연구들은 GD보다 뛰어난 성능을 보인다고 알려져있다. 
% %%그리고, 이 연구는 앞에서 언급했던거와 같이, Global descriptor 연구가 아니기 때문에 우리와 비교 대상이 아님을 다시 한번 노티한다.
% 이 분야는 크게 두 파트로 분류할 수 있는데, 이를 Local Descriptor (LD)~\cite{delf, Teichmann01, Oriane, Weyand01, Donoser01, Iscen_2017_CVPR, Yang01, Teichmann01}와  Global Descriptor (GD)~\cite{Babenko01, Gordo01, Kalantidis01, Weyand01, Babenko03, Radenovic01, SCH01,yang2021dolg, dtop} 로 나뉠 수 있다.
% LD의 연구는 Deep learning 이전에 대표적으로 SIFT~\cite{Lowe01}를 이용하여 image retrieval에 적용해왔다. 
% 이들은 한 이미지당 다수의 feature가 발생되기 때문에, 이들을 aggregation 하는 방법~\cite{Philbin01, JPD+11, TAJ13}을 적용하였다. 
% 이 개념을 Deep learning에 확장한 연구인 DELF~\cite{delf}, DELG~\cite{cao2020unifying}, ASMK을 응용한 연구들~\cite{Teichmann01, tolias2020learning}이 있다. 
% LD 에 비해, GD는 이미지 한장으로부터 단일 Image Feature만을 생성하기 때문에, 상대적으로 효용성이 크다. 
% 특히, GD관련 연구는  CNN backbone으로 부터 추출한 3차원의 feature map에 대해  MAC~\cite{Razavian2015VisualIR}, SPoC~\cite{Babenko03}, CroW~\cite{Kalantidis01}, RMAC~\cite{ToliasSJ15, Gordo01}, GeM~\cite{Radenovic01}같은 다양한 Pooling 기법를 적용하며 진행되어 왔다. 
% 또 다른 방법으로, LD는 GD과 조합하여 사용할 수 있다. 이 같은 연구들은 GD보다 뛰어난 성능을 보인다고 알려져있다. 
% 하지만 이방법은 GD를 통해 Top-K를 찾고, 그 안에서 LD로 re-ranking을 하기 때문에 검색 비용이 많이든다.
% %Top-K만 하는 이유는 Query와 모든 DB사의 거리 측정은 매우 큰 비용이 들기 때문이다.
% %그리고, 이 연구는 앞에서 언급했던거와 같이, Global descriptor 연구가 아니기 때문에 우리와 비교 대상이 아님을 다시 한번 노티한다.
% %

%------------------------------------------------------------------------------

\paragraph{Detect-to-Retrieve ($\mathbf{D2R}$)}

Research on $\mathbf{D2R}$ has been relatively limited in the deep learning field, largely because it necessitates an initial object detection or localization step. This two-stage D2R approach often incurs higher costs for training set construction and learning end-to-end methods. For this reason, there are only a few studies~\cite{Mei01, Salvador01, Chen01, Kucerfashion, Yining01} compared to the ones described above. Nevertheless, the main reason for applying this method is its search accuracy by focusing solely on object-specific features while removing the background noise. 
%These techniques have found applications across various domains, including landmarks~\cite{Mei01, Salvador01, Chen01, Liao01}, fashion~\cite{Mei01, Salvador01, Chen01}, and leaf disease~\cite{leaf01}. 
In addition to the two-stage approach, there are studies that use end-to-end learning. Among them, DIR~\cite{Gordo01} employs RMAC-based pooling, but it does so without utilizing a detection method, opting instead for predefined fixed regions. This approach leverages the region proposal network (RPN) from Faster-RCNN~\cite{fasterrcnn}, making it more akin to a two-stage method than an end-to-end one. 
\alert{Replaced the sentence before: This approach leverages the regional proposal network (RPN) of Faster-RCNN ~\cite{Gordo01}, which uses location supervision, so it is more of a two-stage approach than an end-to-end approach.  
On the other hand, this study uses a one-stage method in the inference phase.}

Salvador~\etal~\cite{Salvador01} present an approach that is fundamentally end-to-end, but unlike this study, they receive object location information for learning object detection. 
\alert{Replaced the sentence before: Salvador~\etal~\cite{Salvador01} essentially provides 1-stage training and inference method, but it utilizes location supervision for object detection. }
R-ASMK~\cite{Teichmann01} stands out for applying LD post-detection, followed by ASMK, an aggregation method described earlier.
\alert{Replaced the sentence before: R-ASMK [46], from which the name "detect-to-Retrieve" originates, extracts LD of detected regions and subsequently applies ASMK.
It consists of 2-stage training and inference. Moreover, we use location supervsion for object detection like the above studies.
Compared to the above mentioned studies, this study is the worst in terms of efficiency.}
\autoref{tab:rel1} shows the previous studies described above, organized by topic. In this table, the proposed method is shown to propose a novel single-stage method that enables end-to-end $\mathbf{D2R}$ learning without location information (\Th{SelfLoc}), unlike previous studies.
\alert{Replaced the sentence before: In this table, we can see that we propose  1-stage training and inference without location supervisions.
Compared with the previous studies mentioned above, we can see that ours is a more efficient method. } 
\\
\CH{I already mentioned that, unlike previous work, this is an E2E-based D2R without location information. 
I think I mentioned this as a difference from the work of RPN-DIR, Salvador, etc. 
Maybe what you're saying is that I should have emphasized a bigger difference on this (inference:stage1, training:stage2??)}
\iavr{Yes, we need to make clear in related work what stages they have in training/testing and what supervision they use. Other properties like what kind of pooling or post-processing (as you say for R-ASMK~\cite{Teichmann01}) are irrelevant in this D2R paragraph. In this sense:
\begin{itemize}
	\item DIR~\cite{Gordo01} is 2-stage training, 1-stage testing, supervised by bounding boxes that are obtained by an algorithm (in one more stage, hence technically 3-stage training).
	\item Salvador~\etal~\cite{Salvador01} is 1-stage training, 1-stage testing but is using location supervision, in fact from the \emph{test set} (Oxford/Paris queries with bounding boxes and augmentations).
	\item R-ASMK~\cite{Teichmann01}, where the name ``Detect-to-Retrieve'' originates, is 2-stage training, 2-stage testing and uses location supervision from an independent set.
\end{itemize}
Can you update the text accordingly? Also, any papers other than those three? For example, I recall Mopuri and Babu, ``Object Level Deep Feature Pooling for Compact Image Representation'' (2015). And maybe my own work, Simeoni \etal, ``Graph-Based Particular Object Discovery'' (2019). Can you analyze these works as above (stages, supervision? Then, anything else? Or course, our main weakness here is that we do not compare with any of those methods in fair settings.}

\CH{I wrote about the four "alert"s (red sentence) in the above.
If it doesn't suit your intention, please let me know.}

%------------------------------------------------------------------------------
\begin{table}
\centering
\small
\setlength{\tabcolsep}{1.7pt}
\begin{tabular}{lccccccc} \toprule
	{\Th{Method}}                              & {\Th{LD}} & {\Th{GD}} &  \Th{[O]}   &  \Th{D2R} & \Th{SelfLoc}   &  \Th{E2E}  & \Th{Land} \\ 
  \midrule	
      DIR~\cite{Gordo01}                           &           & \ch       &             &           &  & \ch        &  \ch     \\
%      DIR+RPN~\cite{Gordo01}                       &           & \ch       &             &  \ch      &  &            &  \ch     \\
      Salvador~\etal~\cite{Salvador01}             &           & \ch       &             &  \ch      &  & \ch        &  \ch     \\
      AGeM~\cite{gu2018attention}                  &           & \ch       &             &           &  & \ch        &  \ch     \\
	 %CroW~\cite{Kalantidis01}                     &           & \ch       & \ch         &            & &            &  \ch       \\	
      Mei~\etal~\cite{Mei01}                       &           & \ch       & \ch         & \ch      &   &            &  \ch       \\	
	 DELF~\cite{delf}                             &           & \ch       &             &          &   &            &  \ch       \\
      Kucer~\etal~\cite{Kucerfashion}              &           & \ch       &             & \ch      &  &            &        \\
	 DELG~\cite{cao2020unifying}                     & \ch       &           &             &          &  &            &  \ch       \\
	 Tolias~\etal~\cite{tolias2020learning}       & \ch       &           &             &          &   &            &  \ch       \\
      PS-Net~\cite{Yining01}                       &           & \ch       &             & \ch      &  &            &           \\
      %Radenović~\etal~\cite{Radenovi01}             &           & \ch       &             &          &   & \ch        &  \ch       \\
      SOLAR~\cite{Ng01}                            &           & \ch       &             &          &   & \ch        &  \ch       \\
      R-ASMK~\cite{Teichmann01}                    &  \ch      &           &             & \ch      &  & \ch        &  \ch       \\
      GLAM~\cite{SCH01}                            &           & \ch       &             &          &   & \ch        &  \ch      \\
      %DOLG~\cite{yang2021dolg}                     &           & \ch       &             &          &   & \ch        &  \ch      \\
      Zhang~\etal~\cite{Zhang01}                   &           & \ch       &             & \ch      &  &            &  \ch       \\
      Peng~\etal~\cite{leaf01}                   &           & \ch       &             & \ch      &  &            &         \\
      Liao~\etal~\cite{Liao01}                  &           & \ch       &             & \ch      &  &            &  \ch       \\
  \midrule
	 \tb{Ours}                                    &           & \red{\tb{\ch}}       &             & \red{\tb{\ch}}     & \red{\tb{\ch}}  & \red{\tb{\ch}}        &  \red{\tb{\ch}}          \\ 
  \bottomrule
\end{tabular}
\vspace{-8pt}
\caption{Related work on Image Retrieval. \Th{LD}:Local Descriptor. \Th{GD}:Global Descriptor. \Th{D2R}:Detected-to-Retrieval. \Th{[O]}:off-the-shelf (pre-trained on ImageNet). \Th{SelfLoc}:Self Localization (Unsupervised-Learning). \Th{E2E} : End-to-End Training. \Th{Land}:Landmark Datasets}
\label{tab:rel1}
\end{table}
%------------------------------------------------------------------------------


==> tex/sec_related-2.tex <==
\section{Related Works}
\label{sec:relatedworks}

\paragraph{Instance Level Image Retrieval (ILIR)}

The field of image retrieval is generally divided into two parts: local descriptors (LD)~\cite{delf, Teichmann01, Oriane, Weyand01, Donoser01, Iscen_2017_CVPR, Yang01, Teichmann01} and global descriptors (GD)~\cite{Babenko01, Gordo01, Kalantidis01, Weyand01, Babenko03, Radenovic01, SCH01,yang2021dolg, dtop}. Research on LD has been applied to image retrieval before deep learning era, where methods like SIFT~\cite{Lowe01} were frequently employed. Given that multiple features are generated for each image in LD-based approaches, various aggregation methods~\cite{Philbin01, JPD+11, TAJ13} have been applied. Deep learning extensions of these concepts include studies such as DELF~\cite{delf}, DELG~\cite{cao2020unifying}, and those applying ASMK~\cite{Teichmann01, tolias2020learning}. 
In particular, DELF is similar to our work in that it uses spatial attention without location supervision, but differs in that it uses it in LD.
In contrast, GD is more useful as it only generates a single, unified feature from an image, simplifying the retrieval process. 
%GD-focused research has leveraged a variety of pooling techniques—such as MAC~\cite{Razavian2015VisualIR}, SPoC~\cite{Babenko03}, CroW~\cite{Kalantidis01}, RMAC~\cite{ToliasSJ15, Gordo01}, and GeM~\cite{Radenovic01}—to extract meaningful information from the three-dimensional feature map extracted from the CNN backbones.
GD focused research has leveraged a variety of pooling techniques~\cite{Razavian2015VisualIR, Radenovic01, Babenko03, Kalantidis01, ToliasSJ15, Gordo01, Radenovic01} to extract meaningful information from the three-dimensional feature map extracted from the CNN backbones. 
Alternatively, some studies have attempted to combine LDs and GDs, achieving performance that surpasses GD alone approaches. However, these hybrid methods come with a drawback: they are computationally expensive. 
%They typically identify the top-k matches using GD and then re-rank these using LD, leading to higher search costs.
They identify the top-k matches using GD and then re-rank these using LD, leading to higher search costs.
% %이 분야는 크게 두 파트로 분류할 수 있는데, 이를 Global Descriptor (GD)~\cite{Babenko01, Gordo01, Kalantidis01, Weyand01, Babenko03, Radenovic01, SCH01,yang2021dolg, dtop} 와 Local Descriptor (LD)~\cite{delf, Teichmann01, Oriane, Weyand01, Donoser01, Iscen_2017_CVPR, Yang01, Teichmann01}로 나뉠 수 있다.
% %LD 에 비해, GD는 이미지 한장으로부터 단일 Image Feature만을 생성하기 때문에, 상대적으로 효용성이 크다. 
% %특히, GD관련 연구는  CNN backbone으로 부터 추출한 3차원의 feature map에 대해  MAC~\cite{Razavian2015VisualIR}, SPoC~\cite{Babenko03}, CroW~\cite{Kalantidis01}, RMAC~\cite{ToliasSJ15, Gordo01}, GeM~\cite{Radenovic01}같은 다양한 Pooling 기법를 적용하며 진행되어 왔다. 
% %LD의 연구는 Deep learning 이전에 대표적으로 SIFT~\cite{Lowe01}를 이용하여 image retrieval에 적용해왔다. 
% %이들은 한 이미지당 다수의 feature가 발생되기 때문에, 이들을 aggregation 하는 방법~\cite{Philbin01, JPD+11, TAJ13}을 적용하였다. 
% %이 개념을 Deep learning에 확장한 연구인 DELF~\cite{delf}, DELG~\cite{cao2020unifying}, ASMK을 응용한 연구들~\cite{Teichmann01, tolias2020learning}이 있다. 
% %또 다른 방법으로, LD는 GD과 조합하여 사용할 수 있다.
% %이는 검색 비용이 많이 들기 때문에, GD를 통해 Top-K를 찾고, 그 안에서 LD로 re-ranking을 한다. 
% %%Top-K만 하는 이유는 Query와 모든 DB사의 거리 측정은 매우 큰 비용이 들기 때문이다.
% %이 같은 연구들은 GD보다 뛰어난 성능을 보인다고 알려져있다. 
% %%그리고, 이 연구는 앞에서 언급했던거와 같이, Global descriptor 연구가 아니기 때문에 우리와 비교 대상이 아님을 다시 한번 노티한다.
% 이 분야는 크게 두 파트로 분류할 수 있는데, 이를 Local Descriptor (LD)~\cite{delf, Teichmann01, Oriane, Weyand01, Donoser01, Iscen_2017_CVPR, Yang01, Teichmann01}와  Global Descriptor (GD)~\cite{Babenko01, Gordo01, Kalantidis01, Weyand01, Babenko03, Radenovic01, SCH01,yang2021dolg, dtop} 로 나뉠 수 있다.
% LD의 연구는 Deep learning 이전에 대표적으로 SIFT~\cite{Lowe01}를 이용하여 image retrieval에 적용해왔다. 
% 이들은 한 이미지당 다수의 feature가 발생되기 때문에, 이들을 aggregation 하는 방법~\cite{Philbin01, JPD+11, TAJ13}을 적용하였다. 
% 이 개념을 Deep learning에 확장한 연구인 DELF~\cite{delf}, DELG~\cite{cao2020unifying}, ASMK을 응용한 연구들~\cite{Teichmann01, tolias2020learning}이 있다. 
% LD 에 비해, GD는 이미지 한장으로부터 단일 Image Feature만을 생성하기 때문에, 상대적으로 효용성이 크다. 
% 특히, GD관련 연구는  CNN backbone으로 부터 추출한 3차원의 feature map에 대해  MAC~\cite{Razavian2015VisualIR}, SPoC~\cite{Babenko03}, CroW~\cite{Kalantidis01}, RMAC~\cite{ToliasSJ15, Gordo01}, GeM~\cite{Radenovic01}같은 다양한 Pooling 기법를 적용하며 진행되어 왔다. 
% 또 다른 방법으로, LD는 GD과 조합하여 사용할 수 있다. 이 같은 연구들은 GD보다 뛰어난 성능을 보인다고 알려져있다. 
% 하지만 이방법은 GD를 통해 Top-K를 찾고, 그 안에서 LD로 re-ranking을 하기 때문에 검색 비용이 많이든다.
% %Top-K만 하는 이유는 Query와 모든 DB사의 거리 측정은 매우 큰 비용이 들기 때문이다.
% %그리고, 이 연구는 앞에서 언급했던거와 같이, Global descriptor 연구가 아니기 때문에 우리와 비교 대상이 아님을 다시 한번 노티한다.
% %

%------------------------------------------------------------------------------

\paragraph{Detect-to-Retrieve ($\mathbf{D2R}$)}

Research on $\mathbf{D2R}$ has been relatively limited in the deep learning field, largely because it necessitates an initial object detection or localization step. This two-stage D2R approach often incurs higher costs for training set construction and learning end-to-end methods. For this reason, there are only a few studies~\cite{Mei01, Salvador01, Chen01, Kucerfashion, Yining01} compared to the ones described above. Nevertheless, the main reason for applying this method is its search accuracy by focusing solely on object-specific features while removing the background noise. 
%These techniques have found applications across various domains, including landmarks~\cite{Mei01, Salvador01, Chen01, Liao01}, fashion~\cite{Mei01, Salvador01, Chen01}, and leaf disease~\cite{leaf01}. 

In addition to the 2-stage approach, there are studies that use end-to-end learning. Among them, DIR~\cite{Gordo01} employs RMAC-based pooling, but it does so without utilizing a detection method, opting instead for predefined fixed regions. This approach leverages the regional proposal network (RPN) of Faster-RCNN ~\cite{Gordo01}, which uses location supervision, so it is more of a two-stage approach than an end-to-end approach.  
On the other hand, this study uses a 1-stage method in the inference phase.

Salvador~\etal~\cite{Salvador01} essentially provides 1-stage training and inference method, but it utilizes location supervision for object detection.

R-ASMK [46], from which the name "Detect-to-Retrieve" originates, extracts LD of detected regions and subsequently applies ASMK.
It consists of 2-stage training and inference. Moreover, it uses location supervision for object detection like the above studies.
Compared to the above mentioned studies, this study is the worst in terms of efficiency.

\autoref{tab:rel1} shows the previous studies described above, organized by topic. In this table, we can see that, unlike previous studies, we propose a novel method that supports 1-stage training, indexing and inference, as well as allowing end-to-end $\mathbf{D2R}$ learning without location supervision. Compared with the previous studies, ours is a more efficient method. 

\iavr{We need to make clear in related work what stages they have in training/testing and what supervision they use. 
\begin{itemize}
	\item DIR~\cite{Gordo01} is 2-stage training, 1-stage testing, supervised by bounding boxes that are obtained by an algorithm (in one more stage, hence technically 3-stage training).
	\item Salvador~\etal~\cite{Salvador01} is 1-stage training, 1-stage testing but is using location supervision, in fact from the \emph{test set} (Oxford/Paris queries with bounding boxes and augmentations).
	\item R-ASMK~\cite{Teichmann01}, where the name ``Detect-to-Retrieve'' originates, is 2-stage training, 2-stage testing and uses location supervision from an independent set.
\end{itemize}
Any papers other than those three? For example, I recall Mopuri and Babu, ``Object Level Deep Feature Pooling for Compact Image Representation'' (2015). And maybe my own work, Simeoni \etal, ``Graph-Based Particular Object Discovery'' (2019). Can you analyze these works as above (stages, supervision? Then, anything else? Or course, our main weakness here is that we do not compare with any of those methods in fair settings.}

\CH{I wrote about the four "alert"s (red sentence) in the above. If it doesn't suit your intention, please let me know.}
\iavr{I have seen it. As I say in another comment just below, I am keeping here my original comment until I revise the section---because there is more to be written.}

\iavr{Thanks for your edits. I am keeping my original comment here to use when I revise this section thoroughly. Then I will remove it. In the meantime, it will help if you can add more papers like those I mention above.}

%------------------------------------------------------------------------------
\begin{table}
\centering
\small
\setlength{\tabcolsep}{1.7pt}
\begin{tabular}{lccccccc} \toprule
	{\Th{Method}}                              & {\Th{LD}} & {\Th{GD}} &  \Th{[O]}   &  \Th{D2R} & \Th{SelfLoc}   &  \Th{E2E}  & \Th{Land} \\ 
  \midrule	
      DIR~\cite{Gordo01}                           &           & \ch       &             &           &  & \ch        &  \ch     \\
%      DIR+RPN~\cite{Gordo01}                       &           & \ch       &             &  \ch      &  &            &  \ch     \\
      Salvador~\etal~\cite{Salvador01}             &           & \ch       &             &  \ch      &  & \ch        &  \ch     \\
      AGeM~\cite{gu2018attention}                  &           & \ch       &             &           &  & \ch        &  \ch     \\
	 %CroW~\cite{Kalantidis01}                     &           & \ch       & \ch         &            & &            &  \ch       \\	
      Mei~\etal~\cite{Mei01}                       &           & \ch       & \ch         & \ch      &   &            &  \ch       \\	
	 DELF~\cite{delf}                             &           & \ch       &             &          &   &            &  \ch       \\
      Kucer~\etal~\cite{Kucerfashion}              &           & \ch       &             & \ch      &  &            &        \\
	 DELG~\cite{cao2020unifying}                     & \ch       &           &             &          &  &            &  \ch       \\
	 Tolias~\etal~\cite{tolias2020learning}       & \ch       &           &             &          &   &            &  \ch       \\
      PS-Net~\cite{Yining01}                       &           & \ch       &             & \ch      &  &            &           \\
      %Radenović~\etal~\cite{Radenovi01}             &           & \ch       &             &          &   & \ch        &  \ch       \\
      SOLAR~\cite{Ng01}                            &           & \ch       &             &          &   & \ch        &  \ch       \\
      R-ASMK~\cite{Teichmann01}                    &  \ch      &           &             & \ch      &  & \ch        &  \ch       \\
      GLAM~\cite{SCH01}                            &           & \ch       &             &          &   & \ch        &  \ch      \\
      %DOLG~\cite{yang2021dolg}                     &           & \ch       &             &          &   & \ch        &  \ch      \\
      Zhang~\etal~\cite{Zhang01}                   &           & \ch       &             & \ch      &  &            &  \ch       \\
      Peng~\etal~\cite{leaf01}                   &           & \ch       &             & \ch      &  &            &         \\
      Liao~\etal~\cite{Liao01}                  &           & \ch       &             & \ch      &  &            &  \ch       \\
  \midrule
	 \tb{Ours}                                    &           & \red{\tb{\ch}}       &             & \red{\tb{\ch}}     & \red{\tb{\ch}}  & \red{\tb{\ch}}        &  \red{\tb{\ch}}          \\ 
  \bottomrule
\end{tabular}
\vspace{-8pt}
\caption{Related work on Image Retrieval. \Th{LD}:Local Descriptor. \Th{GD}:Global Descriptor. \Th{D2R}:Detected-to-Retrieval. \Th{[O]}:off-the-shelf (pre-trained on ImageNet). \Th{SelfLoc}:Self Localization (Unsupervised-Learning). \Th{E2E} : End-to-End Training. \Th{Land}:Landmark Datasets}
\label{tab:rel1}
\end{table}
%------------------------------------------------------------------------------

\iavr{``Attention-based pooling'', possibly to add if a comparison works:
\begin{enumerate}
	\item Lee \etal ``Set Transformer: A Framework for Attention-based Permutation-Invariant Neural Networks'' (2019).
	\item Zhai \etal ``Scaling Vision Transformers'' (2021).
	\item Touvron \etal ``Augmenting Convolutional networks with attention-based aggregation'' (2021).
	\item Psomas \etal ``Keep It SimPool: Who Said Supervised Transformers Suffer from Attention Deficit?'' (2023) (my work).
	\item The ResNet encoder of CLIP.
\end{enumerate}
}

